A Stable and Efficient Covariate-Balancing Estimator for Causal Survival Effects

We propose an empirically stable and asymptotically efficient covariate-balancing approach to the problem of estimating survival causal effects in data with conditionally-independent censoring. This addresses a challenge often encountered in state-of-the-art nonparametric methods: the use of inverses of small estimated probabilities and the resulting amplification of estimation error. We validate our theoretical results in experiments on synthetic and semi-synthetic data.

==> preambles/style <==
%======================== Required packages ========================%
\usepackage{wrapfig}
\usepackage{amssymb, amsmath, amsthm}
\usepackage{dsfont, mathrsfs, color, bm, bbm, enumitem, url}
\usepackage{subfigure, graphicx, transparent, booktabs} 
\usepackage{multirow, titlecaps, accents, makebox, epstopdf, mathtools}
\usepackage{caption}
\usepackage[dvipsnames]{xcolor}
%========================== Figures Path ===========================%
\graphicspath{{graph/}}

%===================== Algorithm Environments ======================%
\usepackage{algorithm, algorithmic}
\renewcommand{\algorithmicrequire}{\textbf{Input:}} 
\renewcommand{\algorithmicensure}{\textbf{Output:}}

% ================== Margins & Layout =================================
\addtolength{\voffset}{0cm} 
\addtolength{\textheight}{1cm} 
\addtolength{\hoffset}{-2cm}
\addtolength{\textwidth}{4cm}

\setlength{\parskip}{1mm}
\linespread{1.12}

%====================== Theorem Environments =======================%
\theoremstyle{definition}
\newtheorem{theorem}{Theorem}[section]
\newtheorem{definition}[theorem]{Definition}
\newtheorem{assumption}[theorem]{Assumption}
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{remark}[theorem]{Remark}
\newtheorem{example}[theorem]{Example}

%========================== NIPS packages ==========================%
\usepackage[utf8]{inputenc}    % allow utf-8 input
\usepackage[T1]{fontenc}       % use 8-bit T1 fonts
\usepackage{url}               % simple URL typesetting
\usepackage{booktabs}          % professional-quality tables
\usepackage{amsfonts}          % blackboard math symbols
\usepackage{nicefrac}          % compact symbols for 1/2, etc.
\usepackage{microtype}         % microtypography

%========== Cross referencing ===========%
\usepackage{xr}
\makeatletter
\newcommand*{\addFileDependency}[1]{% argument=file name and extension
  \typeout{(#1)}
  \@addtofilelist{#1}
  \IfFileExists{#1}{}{\typeout{No file #1.}}
}
\makeatother
 
\newcommand*{\myexternaldocument}[1]{%
    \externaldocument{#1}%
    \addFileDependency{#1.tex}%
    \addFileDependency{#1.aux}%
}

% CODE SNIPPETS

\definecolor{strings}{rgb}{.624,.251,.259}
\definecolor{keywords}{rgb}{.224,.451,.686}
\definecolor{comment}{rgb}{.322,.451,.322}

\usepackage{minted}
\newminted{python}{fontsize=\footnotesize,mathescape=True,escapeinside=@@}

% USEFUL COMMANDS

\newcommand{\pp}{\textcolor{Plum}{\P\,}}
\newcommand{\q}[1]{\red{{\sf Q | #1}}}
\newcommand{\draftdisclaimer}{\begin{center}\begin{framed} DRAFT: DO
NOT CITE OR DISTRIBUTE \end{framed}\end{center}}

% BIBLIOGRAPHY AND LINKS

\usepackage{natbib}
\usepackage[colorlinks,linktoc=all]{hyperref}
\usepackage[all]{hypcap}
\hypersetup{citecolor=MidnightBlue}
\hypersetup{linkcolor=MidnightBlue}
\hypersetup{urlcolor=MidnightBlue}

\usepackage[nameinlink]{cleveref}
\crefname{section}{§}{§§}
\Crefname{section}{§}{§§}
\creflabelformat{equation}{#2\textup{#1}#3}  % <- remove parenthesis from equations


==> sections/32_new.tex <==
\subsection{Augmented Minimax Linear Estimation (AMLE) of $\gamma$}

\khiem{
outlines:
\begin{enumerate}
\item Relate the weight gamma to the Riesz representer. (Done)
\item Give intuitive explanation of gamma
\item Discuss that solving the Riesz via the omega term is unstable.
\item Therefore, solve the Riesz by method of moments and the balancing equation. 
\end{enumerate}
This is somewhat insufficient in relating our approach to AMLE, we will have to ask David about this.
}

In Equation~\ref{eq:riesz-rep-explicit}, we characterized the derivative $d\psi(\hat\lambda)$ explicitly in terms of the survival curve $\hat S$ induced by the hazard $\hat\lambda$. However, due to the missing problem in causal inference, we are only able to estimate that term using observable data and thus the estimator $\gamma$ was introduced. We call this the Riesz representer of the $d\psi(\hat\lambda)$ term: because $d\psi(\hat\lambda)$ is a \textit{continuous linear functional}, the existence of $\gamma$ is implied from the Riesz representation theorem. 

The form of the Riesz representer $\gamma$ in equation \eqref{eq:riesz} inverse probability weighting to replace evaluation of $\delta$ at $A=a$ with an inverse probability weighted indicator; in effect, the indicator identifies the correct population on which to evaluate $\delta$, i.e $\mathbf{1}(E=1,A=a)\delta(A,X)=\mathbf{1}(E=1,A=a)\delta(a,X)$, and weighting corrects for the population selection induced by this indicator. This is typical of Riesz representations in causal and missing data problems. 

However, this Riesz representation cannot be used directly because it depends on the (unknown) inverse probability weights $\omega$. One approach is to estimate the functions $\pi$ and $H$ and simply plug them in to the formula. Doing this yields the one-step estimator \citep[among others]{kennedy2022semiparametric,diaz2020machine,chernozhukov2017double}. However, these methods can be unstable in practice as they often involve estimating inversions (refer to Section \ref{sec:challenge} for more details).

Another approach is to focus on what the weights $\gamma$ \emph{do}, more specifically, its implicit form. First, we can further generalize Equation \eqref{eq:ideal} to be
\begin{equation} 
\label{eq:sample-balance}
\sum_{i=1}^n \sum_{u \le t} \hat r_u(a,X) \delta_u(1,1,X) \\
\approx \sum_{i=1}^n \sum_{u \le t} \hat r_u(a,X) \one(\td T \ge u,A=a)\omega_u(a,X) \delta_u(E_i,A_i,X_i).
\end{equation}
Approximately solving this for a large set of functions $\delta$ yields a \emph{method of moments} estimator for the inverse probability weights $\omega$ and consequently the Riesz representation $\gamma_{\hat\lambda}$ \citep{chernozhukov2022locally}. We will use a regularized method-of-moments approach in which we ask for weights that are (i) not too large and (ii) ensure the approximation \eqref{eq:sample-balance} holds well uniformly over the unit ball of some norm $\norm{\cdot}_{\mathcal{M}}$. In particular, we choose weights by solving the following optimization problem.
\begin{equation}
\label{eq:weight-optimization}
\begin{aligned}
\hat\omega &= \operatorname*{argmin}_{\omega \in \R^{nt}} I(\omega)^2 + \frac{\sigma^2}{nt}\sum_{iu} \omega_{iu}^2 \quad \text{where } \\
I(\omega) &= \max_{\substack{\norm{\delta_u}_\mathcal{M} \le 1 \\ u \in 1 \ldots t}}  \frac{1}{n}\sum_{i=1}^n \sum_{u \le t} \hat r_u(a,X) \delta_u(1,1,X) -
 \frac{1}{n}\sum_{i=1}^n \sum_{u \le t} \hat r_u(a,X) \one(\td T \ge u,A=a)\omega_{iu} \delta_u(E_i,A_i,X_i).
 \end{aligned}
\end{equation}
The final step is to choose the aforementioned norm $\norm{\cdot}_{\mathcal{M}}$. If we consider the role played by these weights in our approximation of the derivative term (see Equation~\ref{eq:derivative-term}), we see that we want \eqref{eq:sample-balance} to hold a single vector-valued function:
our error $\delta=\hat\lambda-\lambda$ in estimating the hazard; we can therefore think of the unit ball $\mathcal{M}$ of our norm as 
a \emph{model} for this error function. In particular, if our model is correct in the sense that $\hat\lambda-\lambda \in \mathcal{M}$,
then the maximal approximation error $I(\omega)$ bounds the approximation error
\begin{equation} 
\label{eq:sample-balance}
\frac{1}{n}\sum_{i=1}^n \sum_{u \le t} \hat r_u(a,X) \delta_u(1,1,X) \\
\approx \frac{1}{n}\sum_{i=1}^n \sum_{u \le t} \hat r_u(a,X) \one(\td T \ge u,A=a)\omega_u(a,X) \delta_u(E_i,A_i,X_i).
\end{equation}
%and moreover generally, as a consequence of linearity,
%\begin{equation}
%Version with \lVert \hat\lambda - \lambda \rVert_{\mathcal{M}} %multiplying the max imbalance.
%\end{equation}
As usual, a natural tradeoff in choosing this model---if we take it to be too small,
this norm will be large or even infinite; on the other hand if we take it to be too large
we will not be able to find weights for which the approximation \eqref{eq:sample-balance} is very accurate for all functions in $\mathcal{M}$.
Choosing our norm $\lVert \cdot \rVert_{\mathcal{M}}$ so that this model is a \emph{Donsker class}, e.g. by using an RKHS norm,
is a reasonable tradeoff\citep[e.g.,][]{hirshberg2019minimax}. When we do this, our estimator will be asymptotically efficient, i.e. asymptotically normal with negligible bias and optimal variance, if $\lambda$ is in this class and we estimate it via empirical risk minimization with appropriate regularization.
%We summarize this theoretical result and describe a concrete implementation in Section~\ref{sec:method} below.

%\textcolor{red}{If we get to it: Error decomposition: imbalance + noise + second order remainder.}

==> sections/32_old.tex <==
\subsection{Augmented Minimax Linear Estimation (AMLE) of $\gamma$}
{\color{magenta} old 3.2}

\khiem{I'm think we should move the this paragraph to related work}
Suppose we fit $\hat \lambda$ on an auxiliary sample so, for our purposes, we may treat it as a deterministic function.  The derivative $\psi'(\hat\lambda)$ is, if it exists in the appropriate sense, a \emph{continuous linear functional} of its argument $\delta=\hat\lambda-\lambda$.
In particular, it will be continuous in the norm induced by the inner product 
$\langle{f,g\rangle} = \E [\ f(O) \cdot g(O)]$ on functions from $Z=(\tilde T,A,X)$
to $\R^t$.  This implies that the value of this functional $\psi'(\hat\lambda)$ at every argument $\delta$ coincides with the value of the inner product of $\delta$ with a unique vector-valued function $\gamma_{\hat\lambda}$ that we call its Riesz representation.
\begin{equation}
\label{eq:riesz-rep}
\psi'(\hat\lambda)(\delta) = \E [\gamma_{\hat\lambda}(Z) \cdot \delta(Z)] \quad \text{ for all} \quad \delta 
\end{equation}
And while we cannot calculate this expectation without knowledge of the distribution of $Z$, the law of large numbers justifies approximating it by a sample average. Thus, taking $\delta=\hat\lambda-\lambda$, 
\begin{equation}
\label{eq:derivative-term}
\begin{aligned}
\psi(\lambda) 
&\approx \psi(\hat\lambda) + \psi'(\hat\lambda)(\lambda-\hat\lambda)  \\
&= \psi(\hat\lambda) +  \E [\gamma_{\hat \lambda}(Z) \cdot  (\lambda - \hat\lambda)(Z) ]\\
&\approx \psi_n(\hat\lambda) + \frac{1}{n}\sum_{i=1}^n \gamma_{\hat \lambda}(Z_i) \cdot (\lambda - \hat\lambda)(Z_i) 
\end{aligned}
\end{equation}

To derive the estimator \eqref{eq:amle}, we substitute an estimator for the Riesz representation $\gamma_{\hat\lambda}$ and the aforementioned indicator for the element $\lambda_u(Z)$ of $\lambda(Z)$. Recall equation (\ref{eq:balance_ind}) from Section \ref{sec:notation}: if the corresponding element $\gamma_u(Z)$ depends only on $Z^{u}=(\mathbf{1}(\tilde T \ge u),A,X)$, this indicator acts as a proxy for $\lambda_u(Z_i)$.

{\color{magenta} 3.2 should start here}
This is, in fact, the case. We can characterize the derivative $\psi'(\hat\lambda)$ explicitly in terms of the survival curve $\hat S$ induced by the hazard $\hat\lambda$ and then, by solving Equation~\ref{eq:riesz-rep}, its Riesz representation $\gamma_{\hat\psi}$.
\begin{equation}
\label{eq:riesz-rep-explicit}
\begin{aligned}
\psi'(\hat\lambda)(\delta) &= \E \left[\sum_{u \le t} \hat r_u(a,X) \delta_u(1,X)\right] && \text{ for } \quad \hat r_u(a,x) = \hat S_t(a,X)\frac{\hat S_{u-}(a,x)}{\hat S_u(a,x)}; \\
\gamma_{u}(Z)  &= \hat r_u(a,X) \one(\td T \ge u,A=a)\omega_u(a,X) && \text{ for } \quad  
\omega_u(a,X) = \frac{1}{H_u(a,X)P(A=a|X)}. 
\end{aligned}
\end{equation}
This is proven in the appendix. Note that the Riesz representation uses inverse probability weighting to replace evaluation of $\delta$ at $A=1$ with an inverse probability weighted indicator; in effect, the indicator identifies the correct population on which to evaluate $\delta$, i.e $\mathbf{1}(E=1,A=1)\delta(A,X)=\mathbf{1}(E=1,A=1)\delta(1,X)$,
and weighting corrects for the population selection induced by this indicator. This is typical of Riesz representations in causal and missing data problems. 


However, this Riesz representation cannot be used directly because it depends on the (unknown) inverse probability weights $\omega$; we must estimate it. One approach is to estimate the functions $\pi$ and $H$ and simply plug them in to the formula. Doing this yields the one-step estimator \citep[among others]{kennedy2022semiparametric,diaz2020machine,chernozhukov2017double}. However, these methods can be unstable in practice as they often involve estimating inversions (refer to Section \ref{sec:challenge} for more details).


Another approach is to focus on what the weights $\gamma$ \emph{do} --- on the implicit characterization \eqref{eq:riesz-rep} rather than the explicit one \eqref{eq:riesz-rep-explicit}. The law of large numbers implies that the equivalence \eqref{eq:riesz-rep} should hold approximately when we replace expectations with sample averages. That is, for all $\delta$, they satisfy
\begin{equation} 
\label{eq:sample-balance}
\frac{1}{n}\sum_{i=1}^n \sum_{u \le t} \hat r_u(a,X) \delta_u(1,1,X) \\
\approx \frac{1}{n}\sum_{i=1}^n \sum_{u \le t} \hat r_u(a,X) \one(\td T \ge u,A=a)\omega_u(a,X) \delta_u(E_i,A_i,X_i).
\end{equation}
Approximately solving this for a large set of functions $\delta$ yields a \emph{method of moments} estimator
for the inverse probability weights $\omega$ and consequently the Riesz representation $\gamma_{\hat\lambda}$ \citep{chernozhukov2022locally}. We will use a regularized method-of-moments approach in which we ask for weights that
are (i) not too large and (ii) ensure the approximation \eqref{eq:sample-balance} holds well uniformly over the unit ball of some norm $\norm{\cdot}_{\mathcal{M}}$. In particular, we choose weights by solving the following optimization problem.
\begin{equation}
\label{eq:weight-optimization}
\begin{aligned}
\hat\omega &= \operatorname*{argmin}_{\omega \in \R^{nt}} I(\omega)^2 + \frac{\sigma^2}{nt}\sum_{iu} \omega_{iu}^2 \quad \text{where } \\
I(\omega) &= \max_{\substack{\norm{\delta_u}_\mathcal{M} \le 1 \\ u \in 1 \ldots t}}  \frac{1}{n}\sum_{i=1}^n \sum_{u \le t} \hat r_u(a,X) \delta_u(1,1,X) -
 \frac{1}{n}\sum_{i=1}^n \sum_{u \le t} \hat r_u(a,X) \one(\td T \ge u,A=a)\omega_{iu} \delta_u(E_i,A_i,X_i).
 \end{aligned}
\end{equation}
What remains is to choose this norm. If we consider the role played by these weights in our approximation of the derivative term (see Equation~\ref{eq:derivative-term}), we see that we want \eqref{eq:sample-balance} to hold a single vector-valued function:
our error $\delta=\hat\lambda-\lambda$ in estimating the hazard; we can therefore think of the unit ball $\mathcal{M}$ of our norm as 
a \emph{model} for this error function. In particular, if our model is correct in the sense that $\hat\lambda-\lambda \in \mathcal{M}$,
then the maximal approximation error $I(\omega)$ bounds the approximation error
\begin{equation} 
\label{eq:sample-balance}
\frac{1}{n}\sum_{i=1}^n \sum_{u \le t} \hat r_u(a,X) \delta_u(1,1,X) \\
\approx \frac{1}{n}\sum_{i=1}^n \sum_{u \le t} \hat r_u(a,X) \one(\td T \ge u,A=a)\omega_u(a,X) \delta_u(E_i,A_i,X_i).
\end{equation}
%and moreover generally, as a consequence of linearity,
%\begin{equation}
%Version with \lVert \hat\lambda - \lambda \rVert_{\mathcal{M}} %multiplying the max imbalance.
%\end{equation}
As usual, a natural tradeoff in choosing this model---if we take it to be too small,
this norm will be large or even infinite; on the other hand if we take it to be too large
we will not be able to find weights for which the approximation \eqref{eq:sample-balance} is very accurate for all functions in $\mathcal{M}$.
Choosing our norm $\lVert \cdot \rVert_{\mathcal{M}}$ so that this model is a \emph{Donsker class}, e.g. by using an RKHS norm,
is a reasonable tradeoff\citep[e.g.,][]{hirshberg2019minimax}. When we do this, our estimator will be asymptotically efficient, i.e. asymptotically normal with negligible bias and optimal variance, if $\lambda$ is in this class and we estimate it via empirical risk minimization with appropriate regularization.

==> sections/abstract <==
%WHY SHOULD YOU CARE ABOUT THIS PROBLEM
We study the problem of estimating survival causal effects, where the aim is to characterize the impact of an intervention on survival times, i.e., how long it takes for an event to occur. Applications include determining if a drug reduces the time to ICU discharge or if an advertising campaign increases customer dwell time. 
% 
Historically, the most popular estimates have been based on parametric or semiparametric (e.g. proportional hazards) models; however, these methods suffer from problematic levels of bias. 
Recently debiased machine learning approaches are becoming increasingly popular, especially in applications to large datasets. However, despite their appealing theoretical properties, these estimators tend to be unstable because the debiasing step involves the use of the \emph{inverses} of small estimated probabilities---small errors in the estimated probabilities can result in huge changes in their inverses and therefore the resulting estimator. This problem is exacerbated in survival settings where probabilities are a product of treatment assignment and censoring probabilities.
%WHAT WE DID
%
We propose a covariate balancing approach to estimating these inverses directly, sidestepping this problem. The result is an estimator that is stable in practice and enjoys many of the same theoretical properties. In particular, under overlap and asymptotic equicontinuity conditions, our estimator is asymptotically normal with negligible bias and optimal variance. % (this means it is not possible to do statistical inference better than ours)
%We introduce a covariate-balancing estimator that is both stable as well as asymptotically normal when the convergence rate of the nuisance estimators are at least $o(n^{-1/4})$.
%This assumption covers a broad range of machine learning methods, including neural networks.
%
%HOW IT WORKS
%Our proposed estimator is based on the efficient influence function of the treatment-specific survival curves, however we sidestep estimating the propensity weight directly, but estimate the balancing weight via a population balance property.
%
% EXPERIMENTS/THEORY TO BACK UP OUR STORY
Our experiments on synthetic and semi-synthetic data demonstrate that our method has competitive bias and smaller variance than debiased machine learning approaches. % because it is stable to extreme weights.
% We present experimental results on synthetic data that demonstrate the stability of our methods.






%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%NOTES


% However, the form of the semi-parametric efficient estimator involves inverse weights, which is unstable.?


% while the bias resulting from the incorrect misspecification of these models was small relative to the estimator's variance in yesterday's small sample sizes and therefore essentially unproblematic, it tends to be the dominant source of error in the larger samples we see today.

%in the large sample sizes we see today [the inability of these models to capture what the data tells us] is the dominant source 

%Existing methods for estimating survival causal effects [CITE Cox, IPCW] tend to suffer either from problematic levels of bias or instability. In particular, the theoretically optimal ... estimator involves the use of 

% Estimates based on parametric or semiparametric outcome models suffer from bias; it's possible to correct this bias using inverse probability weighting, but the resulting estimators suffer from instability due to the use of extreme (estimated) weights. In particular, while there is theory that tells us the essential form of the optimal estimator, it's very difficult to use in practice: it is highly sensitive to some parameters --- small probabilities --- that it requires us to estimate.

% use of this estimator requires us to estimate

% is known, practical ... lead to these instability problems. These ... are our focus. We propose ...

%but there are practical

%bias-corrected estimators exist, (especially using data-adaptive machine learning methods?), but suffer from instability due to the extreme weights required to render ... comparable.

% tend to require the estimation of large we the inverse 
% involve heavily weighting some observations, resulting in instability.


%estimation corrects for this, but 
%In particular, while the essential form of the optimal estimator is known, practical ... lead to these instability problems. These ... are our focus. We propose ...

%but there are practical


%leaves details to us that we usually screw up.

%times up to an event.

%times up to an event under

%probability of survival up to a given time under different treatments.  
%determine the impact of an intervention on the survival time. 





%arising from lack of overlap. 

%The standard approach of using inverse probability of treatment weighting can be sensitive to model misspecification and lead to high-variance estimates due to extreme weights.

%Survival causal effects are important because XXX, but %existing methods suffer either from lack of statistical %efficiency (like YYY) or from instability/high variance due to lack of %overlap (like inverse propensity weighting)

==> sections/approach.tex <==
\section{Approach}
\label{sec:approach}
%In this section, we aim to give an intuitive and self-contained explanation of our \textit{stable} and \textit{efficient} estimator of the parameter $\psi^{a,t}=\psi(\bar\lambda)$. 
%In the first part, we derive a particular estimator of $\psi^{a,t}$ based on first-order approximation. This estimator will later be shown to be semi-parametric efficient under appropriate conditions. This estimator requires, in addition to the hazard function, the estimation of an inverse probability weight. Our main contribution is in the second part where we propose a stable estimator of this inverse probability weight without doing the actual inversion, by looking at its dual view as the Riesz representer of the functional derivative $d\psi^{a,t}(\hat \lambda)$ to be introduced immediately.

\subsection{A first-order approximation and the derivative's Riesz representer}
Given an estimate $\hat \lambda$ of the hazard $\bar\lambda$, (e.g. by using a machine-learning method of our choice to regress $Y^u$ on $X,A,G^u$ at each timestep $u$), the `plug-in estimate' $\psi_n(\hat\lambda)$ is a natural estimate of $\psi(\bar\lambda)$. But we can improve on this using a \emph{first-order correction}. Consider the first-order Taylor expansion of $\psi$ around $\hat \lambda$. In terms of its derivative $d\psi(\hat\lambda)(h)$ at $\hat\lambda$ in the direction $h$,
\begin{equation} \label{eq:expansion}
\psi(\hat\lambda + h) \approx \psi(\hat \lambda) + d\psi(\hat \lambda)(h) \quad \text{ for } h \in \Lambda.
\end{equation}
Taking $h = \bar\lambda-\hat\lambda$, the difference between our actual hazard and our estimate, we get a first-order approximation to our estimand $\psi(\bar\lambda)$. Our main concern will therefore be the estimation of this derivative term $d\psi(\hat\lambda)(\lambda - \hat\lambda)$ where, as established in Lemma \ref{lemma:linearization} in the appendix, 
\begin{equation}
\label{eq:derivative-1}
\begin{aligned}
d\psi(\hat\lambda)(h) &= \E \left[\sum_{u \le t}\hat r_u(X,a) h_u(X,a,1) \right] \quad \text{ for } \quad \hat r_u(X,a) &= -\hat S_t(X,a)\frac{\hat S_{u-}(X,a)}{\hat S_u(X,a)}
\end{aligned}
\end{equation}
\textbf{While $\hat \lambda$ and $\hat r$ are known quantities, derived from our hazard estimate $\hat \lambda$, we will need to substitute something for the \emph{actual} hazard $\bar\lambda$}. For this purpose, $Y_u$ is a natural proxy, as its conditional mean \emph{is} the hazard $\bar\lambda_u(X,A,G)$ at the observed levels of the conditioning variables $X,A,G$; our challenge is make this speak to its value $\bar\lambda_u(X,a,1)$ at often-unobserved levels of those variables. To this end, we observe that the Riesz representation theorem guarantees that, for the space $\Lambda$, there exists a unique element $\gamma$ that acts (via an inner product) on the function $h$ like the functional derivative does, i.e., one satisfying 
\begin{equation}
\label{eq:riesz-rep}
d\psi(\hat \lambda)(h) = \inner{\gamma}{h} = \sum_{u \le t}\E\left[ \gamma_u(X,A,G) h(X,A,G) \right]
\quad \text{ for all } \quad h \in \Lambda
\end{equation}
and, in particular, taking $h=\bar\lambda-\hat\lambda$,
\begin{equation}
d\psi(\hat \lambda)(\lambda-\hat\lambda) = \inner{\gamma}{\lambda-\hat\lambda} = \sum_{u \le t}\E\left[ \gamma_u(X,A,G) \left\{ \bar\lambda(X,A,G)-\hat \lambda(X,A,G) \right\} \right].
\end{equation}
We call $\gamma$ the \textit{Riesz representer} of $d\psi(\hat \lambda)$. Substituting $Y_u$ for $\bar\lambda$ gives us an equivalent expression for our derivative term. By the law of iterated expectations,
\begin{equation}
\label{eq:derivative-2}
\begin{aligned}
d\psi(\hat \lambda)(\lambda - \hat \lambda) &= 
\sum_{u \le t} \E \left [\gamma_u(X,A,G_u) \left\{ \E[Y_u|X,A,G_u] - \hat \lambda_u(X,A,G_u) \right\} \right] \\
&= \sum_{u \le t}  \E\left[\gamma_u(X,A,G_u) \left\{ Y_u - \hat \lambda_u(X,A,G) \right\} \right] \\
\end{aligned}
\end{equation}
So, supposing that we have an estimator $\hat \gamma$ for our Riesz representer, we obtain the following estimator for
$\psi(\bar\lambda)$ by replacing expectations with sample averages as in \eqref{eq:sample-average-approx}.
\begin{equation}
\label{eq:the-generic-estimator}
\hat\psi = \hat\psi_n(\hat\lambda) + \frac{1}{n}\sum_{i=1}^n \sum_{u \le t} \hat \gamma_u(X_i, A_i, G_{i})\left\{ Y^u_i - \hat \lambda_u(X_i, A_i, G_i) \right\}
\end{equation}

\subsection{Estimating the Riesz Representer $\gamma$}
\label{subsec:amle}

$\gamma$ can be characterized in terms of \emph{inverse probability weights}. The explicit solution to the set of equations defining the Riesz representer (Equation~\ref{eq:riesz-rep}) is
\begin{equation}
\begin{aligned}
\label{eq:riesz-rep-explicit}
&\gamma(X,A,G) 
= \frac{\hat r_u(X,a)\one(A=a,G_u=1)}{\E\left[\one(A=a, G_u=1)|X\right]} 
= \hat{r}_u(X,a)\one(A=a,G_u=1)\omega_u(X,a)\\
&\text{ where } \quad
\omega_u(x,a) = \frac{1}{H_{u-}(x,a) \pi(x,a)}
 \text{ and } 
\pi(x,a)=P(A=a \mid X=x).
\end{aligned}
\end{equation}
One approach is to estimate the functions $\pi(x,a)$ and $H_{u-}(x,a)$ appearing in \eqref{eq:riesz-rep-explicit} and assemble them into an estimate $\hat\gamma = \frac{\hat r_u(X,a)\one(A=a,G_u=1)}{\hat H_{u-}(X,a)\hat\pi(X,a)} = \hat r_u(X,a)\one(A=a,G_u=1)\hat\omega_u(X,a)$ of the Riesz representer $\gamma$. Taking this approach yields `one-step' estimator discussed in Section \ref{sec:related-work} below. However, this solution suffers from instability, common in all inverse weight-based estimators. When the ground truth functions $H_{u-}(X,a)$ and $\pi(X,a)$ are very small at some observations, naturally their estimators tends to be very small, hence, slight errors in estimating them can result in large errors in the estimation of their inverses (i.e. $1/(x-\epsilon)-1/x \approx \epsilon/x^2$). Thus, lack of overlap in the data means that such estimators will be unstable, with very large sample sizes needed to get estimates of $\pi$ and $H$ accurate enough to tolerate inversion. Moreover, even when when overlap in the data is not poor, moderate-sized errors in the estimation of $\pi$ and $H$ that occur at smaller sample sizes results in similar issues.  It is common practice to clip these weights to a reasonable range before using them, but ad-hoc clipping often results in problematic levels of bias. In short, we lack practical and theoretically sound methods to make this inversion step work reliably.

Our approach, which avoids this problematic inversion, focuses not on the analytic form of the Riesz representer but on what it does, i.e.,
on the equivalence of the inner product $\smallinner{\gamma}{h}$ to the derivative evaluation $d\psi(\hat\lambda)(h)$. As we lack the ability to analytically evaluate the expectations involved in both, we will use the sample average approximations of these quantities:
$\smallinner{\gamma}{h}_n$ (defined above) and $d\psi_n(\hat\lambda)(h)=\frac{1}{n}\sum_{i=1}^n\sum_{u \le t}\hat r_u(X_i, a) h_u(X_i, a, 1)$.
Inspired by the explicit characterization in \eqref{eq:riesz-rep-explicit}, taking $\hat\gamma$ to have a functional form $\hat\gamma(X_i,A_i,G_i)=\hat r_u(X_i, a) \one(A_i=a, G_{iu}=1) \hat\omega_{iu}$ (for weights $\hat\omega_{iu}$)
, we ask that, for a set of functions $h$,
\begin{equation} 
\label{eq:sample-balance}
\begin{aligned}
\frac{1}{n}\sum_{i=1}^n \sum_{u \le t} \hat r_u(X_i, a)\one(A_i=a, G_{iu}=1) \hat \omega_{iu} h_u(X_i,A_i,G_{iu}) \approx \frac{1}{n}\sum_{i=1}^n \sum_{u \le t} \hat r_u(X_i,a) h_u(X_i,a,1).
\end{aligned}
\end{equation}
In the simpler setting considered in \citet{hirshberg2021augmented}, this approximation has meaning beyond that, suggested by its relationship to the population analog \eqref{eq:riesz-rep}. The quality of the \emph{in-sample approximation} described by \eqref{eq:sample-balance} for the specific function $\hat h=\bar\lambda-\hat\lambda$ is, along with the accuracy of the estimator $\hat\lambda$ and therefore of the linear approximation in \eqref{eq:derivative-1}, one of two essential determinants of the estimator's bias. See Appendix~\ref{sec:sketch}, where we include an informative decomposition of our estimator's error and further discussion.

In light of that, we generalize the approach of \citet{hirshberg2021augmented} for estimating $\gamma$ by ensuring that \eqref{eq:sample-balance} holds for a set $\mathcal{M}$ of hazard-like functions $h$, which we deem as a \emph{model} for function $\hat h = \lambda-\hat\lambda$. In particular, we ask for weights that are (i) not too large, to control our estimator's variance, and (ii) ensure the approximation in Equation (\ref{eq:sample-balance}) is accurate  uniformly over model $\mathcal{M}$. This modeling task is somewhat simplified by the observation that we \emph{only} need a model for $\hat h(X_i,a,1)$, as the presence of the indicator $\one(A_i=a, G_{iu}=1)$ on the right side of \eqref{eq:sample-balance} justifies the substitution of $h_u(X_i,a,1)$ for $h_u(X_i,A_i,G_i)$. Thus, choosing a norm $\norm{\cdot}$ and 
taking the set of vector-valued functions 
$[h_1(x) \ldots h_n(x)]$ with $\sum_u \norm{h_u}^2 \le 1$ as our model for $[\hat h_1(X,a,1) \ldots \hat h_n(X,a,1)]$, we choose weights by solving the following optimization problem
\begin{equation}
\label{eq:weight-optimization}
\begin{aligned}
\hat\omega &= \operatorname*{argmin}_{\omega \in \R^{n|\mc T|}} \left\{ I(\omega)^2 + \frac{\sigma^2}{nt}\sum_{i=1}^n \sum_{u \le t} \hat r_u(X_i, a)^2\one(A_i=a, G_{ui}=1)\omega_{iu}^2 \right\} \quad \text{where } \\
I(\omega) &= \max_{\substack{\sum_{u \le t}\norm{h_u}^2 \le 1 }}  \frac{1}{n}\sum_{i=1}^n \sum_{u \le t} \Big\{\hat r_u(X_i, a) h_u(X_i) -
\hat r_u(X_i,a)\one(A_i=a, G_{iu}=1)\omega_{iu} h_u(X_i)\Big\}.
\end{aligned}
\end{equation}
What remains is to choose this norm with the intention $\smallnorm{\hat h_u}$ is small for all $u$. If our model is correct in the sense that $\sum_u \smallnorm{\hat h_u}^2 \le B^2$, then $B$ times the maximal approximation error $I(\hat\omega)$ bounds the approximation error in \eqref{eq:sample-balance}.

As usual, there is a natural trade-off in choosing this model---if we take it to be too small, $\smallnorm{\hat h_u}$ will be large or even infinite; on the other hand if we take it to be too large, we will be unable to find weights for which the approximation \eqref{eq:sample-balance} is highly accurate for all functions in the model. Choosing a norm with a unit ball that is a \emph{Donsker class}, e.g. a Reproducing Kernel Hilbert Space (RKHS) norm like the one we use in our experiments, is a reasonable trade-off that is common in the literature on minimax and augmented minimax estimation of treatment effects \citep[e.g.,][]{hirshberg2019minimax, kallus2016generalized}. When we do this, our estimator will be asymptotically efficient, i.e. asymptotically normal with negligible bias and optimal variance, if the hazard functions $f(x)=\bar\lambda_u(x,a,1)$ are in this class and we estimate them via empirical risk minimization with appropriate regularization. We discuss the computational aspects of this problem in Appendix~\ref{sec:weight-optimization-details}.

\subsection{Asymptotic Efficiency}
In this section, we will discuss the asymptotic behavior of our estimator, giving sufficient conditions for it to be asymptotically efficient.
Throughout, we will assume $\hat\lambda$ is cross-fit, i.e., fit on an auxilliary sample independent of and distributed like our sample.


Our first condition is that it converges faster than fourth-root rate. This ensures the error of our first-order approximation \eqref{eq:expansion}, quadratic in the error $h=\bar\lambda-\hat\lambda$, is asymptotically negligible. 
\begin{assumption} 
\label{ass:rate}
$\norm{\hat\lambda_u(\cdot,a) - \lambda_u(\cdot,a)}_{L_2(P)} = o_p(n^{-1/4})$ for all $u \le t$.
\end{assumption}
Our second condition is that its error is \emph{bounded} in the norm $\norm{\cdot}$ used to define our model. This ensures that the bound on $I(\hat\omega)$ achieved via the optimization in \eqref{eq:weight-optimization} implies a comparable bound on the error of the derivative approximation $\smallinner{\hat\gamma}{h}_n\approx d\psi(\hat\lambda)(h)$ in \eqref{eq:sample-balance}
for the relevant perturbation $h=\bar\lambda-\hat\lambda$.
\begin{assumption} 
\label{ass:strongnorm-bounded}
$\norm{\hat \lambda_u(\cdot, a) - \lambda_u(\cdot, a)} = O_p(1)$ for all $u \le t$.
\end{assumption}
If our model is correctly specified in the sense that $\norm{\lambda_u} < \infty$ for $\forall u$,
a sensibly tuned $\norm{\cdot}$-penalized estimator of $\lambda_u$ will have these two properties \cite[see, e.g.,][Remark 2]{hirshberg2021augmented}.

Our third condition is that we have a sufficient degree of overlap. 
\begin{assumption}
\label{ass:overlap}
$\E[1/P(A=a, \td T \ge u \mid X)] < \infty$
\end{assumption}
This is a substantially weakened version of the often-assumed `strong overlap' condition that $P(A=a, \td T \ge u \mid X)$ is bounded away from zero,
allowing this probability to approach zero for some $X$ as long as it is `typically' elsewhere. 

Our final condition is, for the most part, a constraint on the complexity of our model.
\begin{assumption}
\label{ass:donskerity}
The unit ball $\mathcal{B}=\left\{ h \ : \ \norm{h} \le 1 \right\}$ is Donsker and uniformly bounded in the sense that $\max_{h : \norm{h} \le 1}\norm{h}_{\infty} < \infty$.
Furthermore, $\left\{\frac{h(\cdot)}{P(A=a, \td T \ge u \mid X=\cdot)} \ : \ \norm{h} \le 1 \right\}$ is Donsker for all $u$.
\end{assumption}
The `furthermore' clause here is implied by the first clause if strong overlap holds, as multiplication by 
the inverse probability weight $1/P(A=a, \td T \ge u \mid X=\cdot)$ will not problematically
increase the complexity of the set of functions $h \in \mathcal{B}$ \emph{if those weights are bounded}.
It is also implied by a strengthened version of the first clause, the condition that $\mathcal{B}$ have a bounded uniform entropy integral,
with our weaker overlap requirement of Assumption~\eqref{ass:overlap} \citep[Remark 4]{hirshberg2021augmented}. 
This tends not to be a problematic strengthening, as the unit balls of many norms that are used in this context,
including H\"older and Sobolev norms involving bounds on $s > \operatorname{dimension}(X)/2$ derivatives
and the RKHS norm we use in our experiments, do have bounded uniform entropy integrals \citep{nickl2007bracketing, zhou2002covering}.


We are now ready to state our main theoretical result, which involves the efficient influence function $\phi^{a,t}$ for estimating $\psi^{a,t}$, 
\begin{equation}
\begin{aligned}
\label{eq:eif}
&\phi^{a,t}(O) = S_t(X, a) - \psi^{a,t}(\lambda) + r(X, a) \one(A=a, G_{u}=1)\omega_u(X_i, a) ( Y_u - \lambda_u(X,a) ) \\
&\text{ for } r(X,a) = - S_t(X,a)\frac{S_{u-}(X,a)}{S_u(X,a)} 
\end{aligned}
\end{equation}

\begin{theorem}
\label{thm:efficiency}
Suppose $\hat\lambda$ is a hazard estimator fit on an auxiliary sample and Assumptions~\ref{ass:rate}-\ref{ass:donskerity} are satisfied. 
Then the estimator $\hat\psi$ described in \eqref{eq:the-generic-estimator}, using the Riesz Representer estimate $\hat\gamma$ obtained by solving 
\eqref{eq:weight-optimization} for any fixed $\sigma > 0$, is \emph{asymptotically linear} with influence function $\phi$. That is, it has the asymptotic approximation
$\hat\psi - \psi = \frac{1}{n}\sum_{i=1}^n \phi(O_i) + o_p(n^{-1/2})$.

\end{theorem}
It follows, via the central limit theorem, that under these conditions $\sqrt{n}(\hat\psi - \psi)$ is asymptotically normal with 
mean zero and variance $V=\E\left[ \phi^{a,t}(O)^2\right]$. This justifies a standard approach to inference based on this
asymptotic approximation, i.e., based on the t-statistic $\smash{\sqrt{n}(\hat\psi-\psi)/\hat V^{1/2}}$ being approximately standard normal if 
$\hat V$ is a consistent estimator of this variance $V$.


As usual for estimators involving cross-fitting, 
working with multiple folds and averaging will yield an estimator 
with the same characterization without an auxiliary sample \citep[e.g.,][]{chernozhukov2018double}. The resulting
estimator is asymptotically linear on the whole sample and, having the efficient influence function $\phi$,
is asymptotically efficient.\footnote{There are many equivalent formal descriptions of what asymptotic efficiency means \citep[e.g.,in][Chapter 25]{van2000asymptotic}. In essence, it implies that no estimator can be reliably perform better in asymptotic terms, either in terms of criteria for point estimation like mean squared error 
or in terms of inferential behavior like the power of tests against local alternatives.}

% Move to experiments, where we do describe a specific model.
%\begin{remark}
%The optimization problem \eqref{eq:weight-optimization} we use to estimate the weights can be solved efficiently when our model is an RKHS ball. It is, in essence, a Ridge regression problem; the weights $\hat\omega$ have a closed-form solution in terms of the space's kernel. We discuss this at greater length in the supplemental material.
%\end{remark}

==> sections/approach2.tex <==
\section{Preliminaries and Related Work}
\label{sec:approach}
In this section, we discuss the preliminaries and previous work on estimation methods of the survival causal parameter $\psi^{a,t}$.

\subsection{First order approximation}
Based on proposition \ref{prop:identification}, we can estimate $\psi^{a,t}$ by plugging in an estimate of the hazard $\lambda$. We denote this the \textit{zeroth-order} estimator:
\begin{equation}
\hat\psi_{ZO}^{a,t} = \psi^{a,t}(\hat \lambda)
\end{equation}
where $\hat \lambda$ denotes an estimate of $\lambda$ (e.g. by machine learning methods). We can however improve on this approach. We start with the functional Taylor expansion:
\begin{equation}
\psi^{a,t}(\lambda) = \psi^{a,t}(\hat \lambda) + d\psi^{a,t}(\hat \lambda)(\lambda - \hat \lambda) + R_2
\end{equation}
where $R_2$ is the second-order remainder term, and $d\psi^{a,t}(\hat \lambda)$ is the Gateaux derivative of $\psi^{a,t}$ at $\hat \lambda$ in the direction $\lambda - \hat\lambda$. If $R_2$ is small enough, then a first order-approximation is hopefully a better estimator. Our main concern will therefore be the estimation of the Gateaux derivative, whose analytically detailed derivation is given in the appendix (lemma \ref{lemma:linearization}). We then obtain
\begin{equation}
\label{eq:riesz-rep-explicit}
\begin{aligned}
d\psi^{a,t}(\hat\lambda)(\lambda - \hat \lambda) &= \E_{X} \left[\sum_{u \le t} r_u(a,X) (\lambda_u - \hat \lambda_u)(a,X)\right]\\
\text{ for } \quad r_u(a,X) &= \hat S_t(a,X)\frac{\hat S_{u-}(a,X)}{\hat S_u(a,X)}
\end{aligned}
\end{equation}
Given an estimation $\hat \lambda_u ~ \forall u \le t$, we can estimate $r_u(a,X)$ by lemma \ref{lem:random_censoring}. $\hat \lambda$ and $\hat r$ can be estimated by \textit{imputing} the treatment and history. However, we are still missing the information of ground truth hazard $\lambda$. We can alternatively use
\begin{equation}
\begin{aligned}
\E_{X}[r_u(a, X) \lambda_u(a, X)] &= \E_{X}[r_u(a, X) \E_{E, \td T}[\one(\td T = u, E=1) | \td T \ge u, A=a, X]]\\
&= \E_{X,E,\td T}[r_u(a, X) \one(\td T = u, E=1)]\\
&\approx \sum_{i=1}^n r_u(a, X_i) \one(\td T_i = u, E_i=1),
\end{aligned}
\label{eq:ideal}
\end{equation}
where the second equality is correct \textit{only if we had observed the ideal data in which all treatments are $a$ and all time $\td T \ge u$.}, for all $X$ in our dataset. This is the missing problem in causal inference and requires us to estimate this term using only observable data.

% {\color{magenta} Mai: maybe put the formula for Riesz here or some introduction context. Riesz representation can be introduced right at the end of Section 3.1}

% the paper optimizes for a function $\hat\gamma$ with the property that \khiem{riesz, mean squared continuous functional}
% \[ \langle\hat\gamma, v \rangle \approx \psi'(\hat\mu)(v) \]
% for all $v$ in some set that hopefully contains $\mu-\hat\mu$ then makes the obvious substitution
% \[ \psi(\mu) \approx \psi(\hat\mu) + \inner{ \hat\gamma}{ \mu - \hat \mu } \]
% Almost. It has to use the proxy $Y$ for $\mu$ because we don't observe $\mu$.  And the inner product that's used here is \khiem{just show 2 expectations are equal}
% \[ \langle u, v \rangle = \E[ u(Z) v(Z)] \] 
% so the Riesz representation is a scalar-valued function,
% and the expectation must be approximated by a sample average.

% {\color{magenta} Mai: the following paragraph seems out of place compared to the context above.}
% Continue giving the intuition behind AMLE. In particular, the idea that we get balance comparable to what we'd get using the actual (unknwon) Riesz representation of the linear functional $\psi'$. In particular, in the case that we're estimating the ATE {\color{magenta} Mai: ??}, that'd be the inverse probability weights.
% \[ L(x) = \langle \gamma_L, x \rangle \]

% {\color{magenta} Mai: don't really understand why L is needed and its context here}

% \khiem{Showing the explicit forms of the weight (both mean outcome and survival outcome) can be another subsection}

% Here, in terms of the dot product on vectors, \khiem{Define the element wise product}
% \[ \langle u, v \rangle = \E[u(X) \cdot v(X)] \]
% so the Riesz representation is a vector valued function. In particular, 
% we are looking at a functional on vector-valued functions with components that are functions of $Z^u$---a linear subspace of the vector-valued functions of $u$---so there exists a Riesz representer \emph{in that subspace}. 



% What we will do here generalizes this approach to this more structured context, in which we are estimating functionals of the hazard---a vector of conditional means given increasing information sets, i.e., given the knowledge that the event has not yet happened at later times.

% We can however compute this term by a \emph{weighted average} of the difference $\lambda$
% $\hat\lambda_u(Z_i)$
% and our proxy $Y_u=\mathbf{1}(E_i=1, \tilde T_i=u)$ for the hazard $\lambda_u(Z_i)$ itself. 
% Something about the Riesz representation based on the dot product blah being ...
% \begin{equation}
% \psi'(\hat\lambda) \cdot (\lambda-\hat\lambda) \approx 
% \frac{1}{n}\sum_{i=1}^n \hat \gamma_i \cdot (Y_i - \hat \lambda(Z_i)) = \frac{1}{n}\sum_{i=1}^n  \sum_{u\le t} \hat\gamma_{iu} \{ \mathbf{1}(E_i=1, \tilde T_i=u) - \hat\lambda_u(Z_i)\}
% \end{equation}

We can however estimate this term using only observable data as follows
\begin{equation}
\begin{aligned}
\E_{X}[r_u(a,X) \lambda_u(a,X)] &= \E_{X,E,A,\td T}[\gamma (X, A,\td T) \one(\td T=u, E=1)]\\
&\approx \sum_{i=1}^n \gamma_u (X_i,A_i,\td T_i) \one(\td T_i=u, E_i=1)\\
\text{  for  } \gamma_u(X,A,\td T) &= r_u(X,a)\frac{\one(\td T\ge u, A=a)}{H_{u-}(X,a)\pi(X,a)}
\end{aligned}
\label{eq:riesz}
\end{equation}

{\color{magenta} Mai: cut this part if too long as well as the derivation of 12 and 13}

This is made possible by the law of iterated expectation\footnote{See appendix for a more detailed explanation}:
\begin{equation}
\begin{aligned}
&\E_{X,E,A,\td T}\left[r_u(X,a)\frac{\one(\td T\ge u,A=a)}{H_{u-}(X,a)\pi(X,a)}\one(\td T=u, E=1)\right]\\
&= \E_{X,E,A,\td T}\left[r_u(X,a)\frac{\one(\td T\ge u, A=a)}{H_{u-}(X,a)\pi(X,a)}\one(\td T=u, E=1)|\one(\td T\ge u),A,X)\right]\\
&= \E_{X}\left[r_u(X,a)\E_{E,\td T}[\one(\td T=u, E=1)|\td T\ge u,A=a,X)]\right]\\
&= \E_{X}[r_u(X,a)\lambda_u(X,a)]\\
\end{aligned}
\end{equation}
The result is the following estimator obtained by an estimation of $\hat\gamma$, which will be further discussed in the next section and \eqref{eq:weight-optimization}.
\begin{equation}
\label{eq:amle}
\hat\psi^{a,t} = \psi^{a,t}_n(\hat\lambda) + \frac{1}{n}\sum_{i=1}^n  \sum_{u\le t} \hat\gamma_{iu} \{ \one(E_i=1, \tilde T_i=u) - \hat\lambda_u(X_i,a)\}
\end{equation}
where $\psi^{a,t}_n(\hat \lambda)=\frac{1}{n}\sum_{i=1}^n \prod_{u \le t}\left( 1- \hat \lambda_u(X_i, a) \right)$ is a sample-based analog of $\psi(\lambda)$.
% This is not an approximation motivated by convenience; it is justified by the \emph{Riesz representation theorem}. 

\input{sections/32_new}

==> sections/experiments.tex <==
\section{Experiments}

We now describe the experimental evidence concerning our estimator. As noted by, e.g., \citet{curth2021survite}, ground truth is almost never  available in causal inference, so synthetic or semi-synthetic data (i.e. synthesized data based on real data) is the standard. We focus on the experiments that provide the most insight into the behavior of our estimator and its competitors; additional experiments and metrics along with implementation details are included in Appendix \ref{sec:experiments_details}.

\subsection{Baselines, Metrics and datasets}
We compare our balancing estimator (\textbf{Balance}) with the outcome regression estimator (\textbf{OR}) and the doubly-robust estimator (\textbf{DR}). We include 2 implementation of \textbf{DR}, one with clipping the weight's denominator to be at least $10^{-3}$ and one without. 

We report the average survival effect at time t: $\Delta^t = \psi^{1,t} - \psi^{0,t}$. Our key error metrics are (1) the relative root-mean-squared-error (\textbf{Relative RMSE}), defined as the RSME of an estimator divided by the RMSE of the \textbf{OR} estimator, which we take to be the baseline, and (2) the Bias over Standard Error ratio (\textbf{Bias/StdE}). Let $\{\hat\Delta^t_q\}_{q=1}^Q$ be our estimates over $Q$ simulations and $\Delta^t$ the ground truth, The RSME, Bias, and Standard Error at time $t$ are defined as $\sqrt{\frac{1}{Q}\sum_q(\hat\Delta^t_q - \Delta^t)^2}, \frac{1}{Q} \sum_q(\hat\Delta^t_q - \Delta^t), \sqrt{\frac{1}{Q}\sum_{q}(\hat\Delta^t_q - \frac{1}{Q}\sum_q \hat\Delta^t_q)^2}$, respectively.

%% R code for probability a random variable is in the usual 99% interval for a standard normal
%% when it's actually normal with mean 1 and 3 (or maybe -1 and -3; doesn't matter) respectively 
%c = qnorm(.995)
%pnorm(c+1)-pnorm(-c+1)
%pnorm(c+3)-pnorm(-c+3)
%[1] 0.9422929
%[1] 0.3357207

%\subsection{Datasets}

We use the two datasets from \citet{curth2021survite} with slight modifications; note that they are concerned with the heterogeneous treatment effect and thus incomparable in our context. For the first dataset \textbf{Synthetic}, we modified the assignment distribution to $a \sim \text{Bern}(\text{Sigmoid}(\xi \times \sum_p x_p))$ where $x$ is a sample of a 10-dimensional multivariate normal, so that $\xi$ controls the lack of overlap from propensity (the higher $\xi$ the less overlap as \text{Sigmoid} saturates quicker). The default value of $\xi$ is $0.3$. We refer readers to the authors' exposition of the different biases arising from censoring and assignment in this dataset. The second dataset \textbf{Twins} is a semi-synthetic dataset based on the Twins dataset \citep{louizos2017causal}. For both, we set $t_{max}=30$. We  use 200 and 500 observations for \textbf{Synthetic} and \textbf{Twins}, respectively, for each $Q=100$ simulations of each experiment. We provide the full data generating process in \ref{sec:implementation}, \ref{sec:datasets}.


\subsection{Discussion of results}
Poor overlap can effect estimators in 2 ways (1) make naive outcome regression estimators biased and (2) lead to extreme numerical inverses in inverse-weight-based estimators. We illustrate this with 2 experiments for censoring bias/poor overlap in time and treatment bias/poor overlap in propensity.
\paragraph{Metrics over time.} From Figure \ref{fig:time}, in both datasets, \textbf{Balance} is both accurate and inferentially useful i.e. we can construct meaningful confidence interval, without suffering from the poor overlap at higher times. \textbf{Balance} has comparable RMSE to \textbf{OR}, where \textbf{DR} and \textbf{DR-clip} are much worse; in \textbf{Twins}, \textbf{DR} clearly runs into large numerical inverses, and \textbf{DR-clip}, despite its improvements, is still far from \textbf{Balance}. Yet, \textbf{Bias/StdE} plots show that \textbf{OR} has serious bias issue that is exacerbated by censoring bias at higher times. This bias is extremely problematic for inference: an \textbf{Bias/StdE} of $1.3$ at time $t=15$ in \textbf{Synthetic} means that a nominal 95\% confidence interval contains the truth only 74.5\% of the time. In contrast, this number is always above 92\% for \textbf{DR} and \textbf{Balance} ($\textbf{Bias/StdE} \le 0.5$), but of course, as seen from \textbf{Relative RMSE} plots, \textbf{DR} and \textbf{DR-clip} have very high standard error that push their RMSE up and thus highly inaccurate.

\begin{figure}[hbt!]
\centering
\includegraphics[width=1.\textwidth]{figures/time.png}
\caption{The effect of lack of overlap in propensity on \textbf{Bias/StdE} and \textbf{Relative RSME}.}
\label{fig:time}
\end{figure}

\paragraph{Metrics over varying propensity.} In Figure \ref{fig:overlap}, we re-run \textbf{Synthetic} for $\xi \in \{0.1, 0.2, 0.3, 0.4, 0.5\}$ and report the metrics at $t=15$ to see how poor overlap from extreme propensities influence our estimators. We observe similar behavior of estimators as seen in the first experiment. As overlap decreases, we see that both \textbf{OR}'s \textbf{Bias/StdE} and \textbf{DR}'s \textbf{Relative RMSE} increase. \textbf{DR-clip} was omitted in \textbf{Synthetic} plots as the estimates here are much less extreme and not truncated. Despite that, because of small sample sizes, we still see the same large errors in \textbf{DR}. In contrast, \textbf{Balance} is very stable across degrees of overlap, again proving its capability to fix \textbf{DR}'s accuracy problem while being less biased than \textbf{OR}, which was also shown in our semi-parametric efficiency theory.

\begin{figure}[htb!]
\centering
\includegraphics[width=0.5\textwidth]{figures/overlap.png}
\caption{The effect of lack of overlap in time on \textbf{Bias/StdE} and \textbf{Relative RSME}.}
\label{fig:overlap}
\end{figure}


==> sections/introduction <==
\section{Introduction}
%\khiem{introduction (add intro plot here, terse description of data more detail in exp), setting (stastical, causal), approach(overlap challenge (add motivation plot here), AMLE, method), related work (refernces, OR and IPW, EIF), Theory and Implementation ?(asymptotic analysis, RKHS, survival estimation, bla), Experiment results.}

Estimating the impact of interventions on survival times is a key objective in numerous studies. This problem is important in various domains, including drug efficacy's evaluation at ICU stay duration and assessment of advertising campaigns' effects on customer dwell time.

The predominant approach for assessing the impact of interventions on survival times is to employ the Cox proportional hazards model (CoxPH) \citep{cox1972regression, andersen1982cox}. This model estimates conditional hazard ratios, which serve as a measure of survival causal effects. However, the causal interpretation of conditional hazard ratios within the CoxPH model can be complex \citep{martinussen2022causality,vansteelandt2022assumption}. Hence, there has been a growing interest in directly estimating \textit{counterfactual survival curves} and consequently deriving survival causal effects from these estimates \citep{westling2023inference} such as the average survival effect, the residual average survival effect, and the survival quantile effect \citep{mansourvar2016additive, mao2018propensity}. A counterfactual survival curve represents the probability of an event occurring at a specific point in time, if contrary to fact, the entire population had undergone a specific intervention, given that the event of interest has not yet occurred. %Some commonly investigated survival causal effects include 

Traditional approaches for estimating counterfactual curves in survival analysis have relied on conditional parametric or semiparametric regression models \citep{kleinbaum2012parametric,cox1972regression}, or weighted methods based on inverse probability of censoring and treatment weighting (IPW) \citep{robins1992recovery}. However, both approaches can suffer from model misspecification i.e. the model does not contain the truth. Weighted methods are also susceptible to extreme inversions \citep{kang2007demystifying,kallus2022optimal,kallus2021more}. In recent years, debiased machine learning approaches have gained popularity due to their appealing double robustness property which deals with model misspecification in addition to being semiparametric efficient \citep{kennedy2022semiparametric}. Specifically, double robustness implies that even if only certain models that need to be estimated are correctly specified, these approaches remain consistent, ie., asymptotically unbiased. Semiparametric efficiency refers to the ability of an estimator or estimation method to achieve the smallest possible \textit{asymptotic} variance among a class of semiparametric estimators. Despite their desirable theoretical properties, debiased machine learning methods \textit{still} face challenges associated with extreme inversions because they are necessarily characterized by inverse probability weights \citep{chernozhukov2022riesznet}.

Covariate balancing methods have been proposed as a solution to the issue of extreme weights encountered in other approaches \citep{ben2021balancing}. 
%TODO: refine (skip)
Instead of directly incorporating inverse probabilities, these methods employ a weight-learning process that yields more stable estimates while preserving crucial properties like semiparametric efficiency. However, the application of these methods to estimate survival causal effects has been significantly limited \citep{xue2023rkhs,wong2017kernel,abraich2022survcaus,johansson2022generalization,santacatterina2023robust,kallus2021optimal,yiu2022joint}, with none of them providing results on asymptotic normality. Asymptotic normality is crucial for statistical inference, hypothesis testing, and the construction of confidence intervals, highlighting a current gap in the literature.

We contribute to the literature of survival causal effects estimation by presenting a novel approach based on covariate balancing techniques. Our proposed method offers stability in practical applications. When certain conditions such as overlap and asymptotic equicontinuity are met, it provides asymptotic normality with minimal bias and optimal variance, ie., statistical efficiency. We substantiate these claims both theoretically and through experiments conducted on synthetic and semi-synthetic data.
Proofs, additional experiments and some technical details are deferred to appendices.


==> sections/junk.tex <==

To address the problem of lack of overlap and weight inversion, we propose \methodname, a balancing estimator based on the EIF. The estimator is both efficient under sufficiently fast rate nuisance estimation and inversion-free. We motivate our approach by parameterizing the EIF in terms of a balancing weight with an associated population balancing equation. 
%Next, we detail our algorithm to estimate $\estimand(t, a)$ by balancing. Finally we make connections to past works that attempted at balancing for survival data and similar.

%\subsection{Balancing EIF}

We parameterize $\eta$ as $(\omega, \lambda)$:
\begin{align*}
&\phi(t, a, \lambda, \omega)(O) = S(t|a,X)\\
&- \sum_{u\le t}S(t|a,X)\frac{S(u-|a,X)}{S(u|a,X)}\one(\td T \ge u,A=a)\omega(u|a,X)\left(\one(\td T=u,E=1)- \lambda(u|a,X)\right)
\end{align*}
A look at \ref{prop:eif} reveals that $\omega(u|a,X) \defeq \frac{1}{H(u|a,X)\pi(a|X)}$. More importantly, $\omega$ satisfies the population balancing equation:
\begin{equation}
\label{eq:balancing}
\E[\one(\td T\ge u, A=a)\omega(u|a,X)f(X)] = \E[f(X)]
\end{equation}
for all bounded $f$ and for each $u \in |\mc T|$ and $a \in \{0, 1\}$. Indeed, we have:
\begin{align*}
\E[\one(\td T\ge u, A=a)\omega(u|a,X)f(X)] &= \E[\E[\one(\td T\ge u,A=a)|X]\omega(u|a,X)f(X)]\\
&= \E[P(\td T\ge u, A=a|X)\omega(u|a,X)f(X)]\\
&= \E[H(u|a,X)\pi(a|X)\omega(u|a,X)f(X)]\\
&= \E[f(X)]
\end{align*}

\section{Asymptotic Analysis}
We now present our main theoretical result: under the primary assumption that the hazard function is estimable at $o(n^{-1/4})$ rate, our covariate balancing estimator is asymptotically linear and efficient with variance equal to the variance of the efficient influence function. We start with the following assumptions.


\begin{assumption} (Rate of the hazard estimator)
$$
\norm{\hat\lambda(t|a,X) - \lambda_0(t|a,X)}_{L_2(P_0)} = o_p(n^{-1/4})\quad \text{and} \quad \norm{\hat\lambda(t|a,X) - \lambda_0(t|a,X)}_{\mc F} = O_p(1) 
$$ for all $a \in \{0, 1\}$ and $t \in \mc T$.
\end{assumption}
beside the consistency rate, we additionally require that the error in $\mc F$-norm is bounded in probability, a requirement from our balancing weight estimation. For example, this requirement wil be satisfied if $\mc F$ is a RKHS.

\begin{assumption} (Characterization of $\mc F$)
\label{ass:F}
Reorder 
\end{assumption}

\begin{assumption} (Strong overlap)
\khiem{@David help with this assumption}
\label{ass:rate_lambda}
There exists $\alpha \in (0, \infty)$ such that $P(\td T \ge u, A=a|X) \ge 1/\alpha$ almost surely.
\end{assumption}

We are now ready to state our main theoretical result.

\begin{theorem}
\label{thm:efficiency}
If assumptions ... hold, then:
$$
\hat\psi(t, a) - \psi_0(t, a) = P_n[\varphi(t,a,\lambda_0,\omega_0)(O_i)] + o(n^{-1/2})
$$
therefore:
$$
\sqrt{n}(\hat \psi(t, a) - \psi_0(t, a)) \Longrightarrow \mc N(0, P_0[\varphi(t,a,\lambda_0,\omega_0)(O_i)^2])
$$
\end{theorem}

\paragraph{Proof sketch.} 

\paragraph{Discussion.}

==> sections/method <==
\section{Theory}
\label{sec:method}
In this section, we continue the remaining task in Section~\ref{sec:approach}, which is to choose the norm $\lVert \cdot \rVert_{\mathcal{M}}$. Our choice of model will be the unit ball of an RKHS with norm $\lVert \cdot \rVert_{\mathcal{M}}$ and bounded kernel.
Essentially, when our hazard function is in our RKHS and we use a cross-fit rate-optimal estimator $\hat\lambda$, our estimator will be asymptotically efficient given strong overlap. 

\begin{assumption} (Rate of the hazard estimator)
\label{ass:rate}
$$
\norm{\hat\lambda_t(a,X) - \lambda_{t}(a,X)}_{L_2(P)} = o_p(n^{-1/4})\quad \text{and} \quad \norm{\hat\lambda_t(a,X) - \lambda_{t}(a,X)}_{\model} = O_p(1) 
$$ for all $a \in \{0, 1\}$ and $t \in \mc T$.
\end{assumption}
A sensibly tuned $\norm{\cdot}_\model$-penalized estimator will have these properties 
when $\norm{\lambda_u}_\model < \infty$ \cite[see, e.g.,][Remark 2]{hirshberg2021augmented}.


\begin{assumption}{(Strong overlap)}
\label{ass:overlap}
There exists $\alpha \in (0, \infty)$ such that $P(\td T \ge u, A=a|X) \ge 1/\alpha$ almost surely.
\end{assumption}
Assumption \ref{ass:overlap} indicates that the survival curve $S$ is continuous in the hazard $\lambda$. More specifically, when overlap is poor, small changes in the hazard can induce large changes in the survival curve, making it impossible to find a \emph{regular} estimator of the survival curve \citep{hirshberg2021augmented}.

\begin{theorem}
\label{thm:efficiency}
Let $\norm{\cdot}_{\model}$ be the norm on an RKHS with kernel $K$ satisfying
$\max_z K(z,z) < \infty$. Then if $\hat\lambda$ is an estimator fit on an auxiliary sample satisfying both Assumption \ref{ass:rate} and \ref{ass:overlap}, the estimator of $\hat \psi$ (through first-order Taylor expansion and the Riesz representer as discussed in Section~\ref{sec:approach}), for any fixed $\sigma > 0$,
is \emph{asymptotically linear},
i.e.,
\[ \hat\psi - \psi = \frac{1}{n}\sum_{i=1}^n \phi(T_i,A_i) + o_p(n^{-1/2}), \] 
with influence function 
\[\phi(t,a) = S_t(a,X) \left(1 - \sum_{u\le t}\frac{S_{u-}(a,X)}{S_u(a,X)}\frac{\one(\td T\ge u,A=a)}{H_u(a,X)\pi(a|X)}\left(\one(\td T=u,E=1) - \lambda_u(a,X)\right)\right) \]
\end{theorem}
Followed by the central limit theorem and Theorem \ref{thm:efficiency}, $\hat\psi - \psi$ is assymtotically normal with variance $\E\left[ \phi(T,A)^2/n\right]$. Consequentially, this justifies a standard approach to inference based on the 
asymptotically-valid approximation, i.e the
t-statistic $(\hat\psi-\psi)/\sqrt{\hat V}$ is standard normal if 
$\hat V$ is an estimator of this variance.

As usual for estimators involving cross-fitting \citep{chernozhukov2018double}, 
working with multiple folds and averaging will yield an estimator 
with the same characterization without an auxilliary sample. The resulting
estimator is asymptotically linear on the whole sample and its influence function
$\phi$ is the efficient influence function, i.e, it is asymptotically efficient.

\begin{remark}
The optimization problem \eqref{eq:weight-optimization} we use to estimate the weights can be solved efficiently when our model is an RKHS ball. It is, in essence, a Ridge regression problem; the weights $\hat\omega$ have a closed-form solution in terms of the space's kernel. We discuss this at greater length in the supplemental material.
\end{remark}


==> sections/preliminaries.tex <==
\section{Setting}
In this section, we review the notations and main quantities in standard discrete survival analysis (Section \ref{sec:discreate_surv_analysis}). We refer interested readers to e.g. Chapter 16 of \cite{crowder2012multivariate} for further details. We then introduce counterfactual survival analysis including the causal parameter of interest and  identification assumptions using the Neyman-Rubin potential outcome framework \citep{neyman1923application, rubin1974estimating} (Section \ref{sec:counterfactual_surv}). Finally, some useful notation is introduced in Section \ref{sec:notation}.

\subsection{Discrete Survival Analysis}
\label{sec:discreate_surv_analysis}
\paragraph{Data structure.} We define an observable survival data unit as the set of random variables $(X, E, \td T)$ where $X \in \mc X \subseteq \R^d$ is the covariate recorded prior to the beginning of the study. To define $E$ and $\td T$, let $T \in \mc T \cup \{\infty\}$ be the time-to-event and $C \in \mc T$ the time-to-censoring (censor time), where $T = \infty$ means that the event has not happened during the study time window $\mc T$. 
In a clinical study, $T$ might be the patient's time from their entry into the study until their ICU discharge - the event of interest. This event might not occur during the time the study is conducted, or the patient might drop out before the end of the study, therefore a censoring time $C$ is introduced. Define $\td T = \min\{ T, C\}$ the right-censored time and $E = \one(T \le C)$ the event indicator. If $E = 1$, the event is observed and occurs at time $\td T = T$, otherwise, the event has not happened or is censored at time $\td T = C$. We assume discrete $\mc T = [\tmax] = \{0,1,..,\tmax\}$, $\tmax \in \mbb Z_+$ and $P(T=0) = 0$, so that zero times are ruled out. Denote by $|\mc T|$ the total number of time points and $|t| = |\{u \in \mc T: u \le t\}|$ the number of time points less than or equal to $t$. $t_{max}$ may be chosen by the user, or as a result of administrative censoring $P(C \le t_{max}) = 1$.

\paragraph{The marginal and sub-survival functions.} We seek to recover the distributions of latent time $T$ from the observable $\td T$ and $E$. Define the marginal-hazard, the marginal-survival function of $T$ and the marginal-censoring function of $C$ as follows:
\begin{equation}
\begin{aligned}
h_t(x) = P(T=t | X=x,T\ge t); \quad S_t(x) = P(T>t|X=x); \quad G_t(x) = P(C>t|X=x).
\end{aligned}
\end{equation}
These definitions imply a one-to-one relationship between $h$ and $S$: letting $t-=\max(0,t-1)$, 
\begin{equation}
h_t(x) = \frac{P(T=t|X=x)}{P(T\ge t|X=x)} = \frac{P(T=t|X=x)}{S_{t-}(x)}; \quad
S_t(x) = S_{t-}(x)(1 - h_t(x)) = \prod_{u \le t} (1-h_u(x)).
\end{equation}
For observable data, define the sub-hazard and sub-survival function as:
\begin{equation}
\lambda_t(x) = P(\td T = t, E=1| X=x,\td T \ge t); \quad
H_t(x) = P(\td T > t | X = x).
\end{equation}
When $T$ and $C$ are conditionally independent given $X$, the following proposition relates the sub-distributions and the marginal-distributions:
\begin{proposition}
If $T \perp C | X$ then: $h_t(x) = \lambda_t(x)$, therefore: 
\begin{equation}
S_t(x) = \prod_{u \le t}(1- h_u(x)) = \prod_{u \le t}(1- \lambda_u(x)).
\end{equation}

Additionally, the sub-survival function decomposes into a product of the marginal-survival functions of the event and censoring: $H_t(x) = S_t(x)G_t(x).$
\label{lem:random_censoring}
\end{proposition}
We provide a proof in Appendix \ref{sec:proof2122}. This equivalence enables the estimation of all identities defined up to now from observable data. From here on, we will use term hazard to refer to the sub-hazard. 


\subsection{Counterfactual Survival Analysis}
\label{sec:counterfactual_surv}
\sloppy\paragraph{Data structure.} We define the ideal data unit in counterfactual survival analysis as $(X, E, A, T(0), T(1), C(0), C(1))$, where $A \in \{0, 1\}$ is a binary random variable indicating e.g. whether or not a patient receives the treatment, $T(a)$ is the event time of interest under $A=a$ and similarly for $C(a)$. With the introduction of $A$, we define $T = AT(1) + (1-A)T(0)$ and $C = AC(1) + (1-A)C(0)$, therefore the observable time $\td T$ and event indicator $E$ are defined as before. The observable data unit is now $O = (X, E, A, \td T)$. In this context, we will talk about the treatment-specific hazard and survival function, $\lambda_t(a,x)$ and $S_t(a,x)$, characterized as in Section \ref{sec:discreate_surv_analysis} in terms of the conditional distribution given treatment $A=a$. With Lemma  \ref{lem:random_censoring}, we then define,
\begin{equation}
\lambda_t(x, a) = P(E=1,\td T = t|X = x, A = a, \td T \ge t); \quad S_t(x, a) =  \prod_{u\le t} (1-\lambda_u(x,a))
\end{equation}
\paragraph{Survival causal parameter of interest: the counterfactual survival function.} We will focus mainly on the counterfactual survival function at time $t \in \mc T$ and treatment $a \in \{0, 1\}$: $\estimand^{a,t} = P(T(a) > t)$. Other commonly encountered parameters can be built from it such as the average survival effect at time $t$: $(\estimand^{1, t} - \estimand^{0, t})$ and the treatment-specific mean survival time $\sum_{t \le t_{max}} \estimand^{a,t}$ as well as its average effect counterpart.
Where convenient, we will write $\estimand$ in place of $\estimand^{a,t}$, letting
the treatment and time of interest be inferred from context.

\paragraph{Identification} To identify the counterfactual survival function using the observable data, similar to \citet{hubbard2000nonparametric, bai2013doubly,bai2017optimal,westling2023inference,diaz2019statistical, cai2020one}, we require the following testable and untestable assumptions:
\begin{itemize}
\item (A1) $T(a), C(a) \perp A \vert X$ for each $a \in \{0, 1\}$.
\item (A2) $T(a) \perp C(a) \vert A=a, X$ for each $a \in \{0, 1\}$.
\item (A3) $P(A=a|X) > 0$ almost surely.
\item (A4) $P(C(a) \geq t|X) > 0 $ positivity (censoring),
\end{itemize}
\begin{proposition}
When Assumptions~(A1)-(A4) hold, $\psi^{a,t}$ can be computed by observable quantities
\begin{equation}\label{eq:identification}
\begin{aligned}
\psi^{a,t} &= \E\left[S_t(X,a)\right] = \E\left[\prod_{u \le t}\left( 1- \lambda_u(X,a) \right)\right].
\end{aligned}
\end{equation}
\label{prop:identification}
\end{proposition}
The proof, along with a discussion of the assumptions, appears in Appendix \ref{sec:proof2122}. 
\subsection{Notation for our proposed approach}
\label{sec:notation}
In the next section, it will be useful to think of the hazard at time $u$, $\lambda_u(a,x)$, as $\bar\lambda_u(x,a,1)$ where 
\begin{equation}
\label{eq:noisy-evaluation}
\begin{aligned}
\bar \lambda_u(x,a,g) 
&= P(E=1, \td T=u |X=x ,A=a, \one(\td T \ge u) = g_u) \\
&= \E[ Y^u \mid X=x, A=a, \one(\td T \ge u) = g_u] \quad && \text{ for } \quad Y^u = \one(E=1, \td T=u). 
\end{aligned}
\end{equation}
Furthermore, we'll think of the functions $\bar\lambda_1 \ldots \bar\lambda_{T}$ as the \emph{components} 
of a vector-valued function $\bar\lambda$ with $[\bar\lambda(x,a,t)]_u = \bar\lambda_u(x,a,\one(t \ge u))$
Note that this vector-valued function has the property that its $u$th component depends on $t$ \emph{only} through the indicator $\one(t \ge u)$;
we will call the space of vector-valued functions with this property the `hazard-like functions' $\Lambda$. And we will think of our
estimand $\psi^{a,t}$, as identified in Proposition \ref{prop:identification}, as a functional $\psi$ on this space $\Lambda$ \emph{evaluated at} $\bar \lambda$:
\begin{equation}
\label{eq:estimand-as-functional}
\psi^{a,t} = \psi(\bar\lambda) \quad \text{ where } \quad \psi(\bar l) =  \E\left[\prod_{u \le t}\left( 1- \bar l_u(X,a,1) \right)\right].
\end{equation}
We've written things in these terms to emphasize the analogy between our estimation problem and the problem of estimating a functional of a conditional 
expectation function considered in \citet{hirshberg2021augmented} and \citet{chernozhukov2022debiased}. What we are estimating is a functional of a vector-valued function $\bar\lambda \in \Lambda$ that is, 
in each component, the conditional expectation function of an observed outcome $Y^u$ given observed conditioning variable $\{ X,A,\one(\td T \ge u) \}$. 
We will work with an inner product on this space $\Lambda$ defined in terms of a random variable $X,A,\td T$ with the same distribution as $(X_1,A_1,\td T_1)\ldots (X_n,A_n,\td T_n)$.\footnote{Note that this is an average over $X,A,\td T$ \emph{only}. If $\hat f$ and $\hat g$ are random variables, $\inner{\hat f}{\hat g}_t$ will be the random variable $\E[\sum_{u \le t} \hat f_u(X,A,G^u) \hat g_u(X,A,G^u) \mid \hat f, \hat g ]$. We will do this conditioning implicitly throughout.} Letting $G^u=\one(\td T \ge u)$ here and below,
\begin{equation}
\inner{f}{g} = \E \left[\sum_{u \le t} f_u(X,A,G^u) g_u(X,A,G^u)\right] \quad \text{ for } \quad f, g \in \Lambda.
\end{equation}
\khiem{drop this}
While we cannot evaluate the functional $\psi$ or the inner product $\inner{\cdot}{\cdot}$ exactly because we do not know the distribution of $(X,A,\tilde T)$, natural sample-average approximations are available.
\begin{equation}
\label{eq:sample-average-approx}
\begin{aligned}
\psi_n(\bar l) =  \frac1n \sum_{i=1}^n \left[\prod_{u \le t}\left( 1- \bar l_u(X_i,a,1) \right)\right]; ~ \inner{f}{g}_n = \frac1n\sum_{i=1}^n \left[ \sum_{u \le t} f_u(X,A,G^u) g_u(X,A,G^u) \right]
\end{aligned}
\end{equation}

==> sections/relatedwork <==
\section{Related works}
%graham pinto and egel: https://www.nber.org/papers/w13981


%survival analysis
%parametric and semiparametric methods

%ipcw

\paragraph{Estimation of the survival functions.} The Cox proportional hazard (CoxPH) model \cite{cox1972regression, andersen1982cox}, has long been regarded as the standard model in survival analysis, and more recently, deep learning approaches have been proposed to leverage the Cox PH framework for survival analysis tasks. % What do these look like?
There have been proposed methods in survival analysis that utilize deep learning techniques based on the CoxPH model. Among others \cite{zhu2016deep,katzman2018deepsurv,faraggi1995neural,wang2021cox,ching2018cox,sun2020genome, zhong2022deep,nagpal2021deepcoxmixtures,meixide2022neural,lv2022transsurv,tibshirani1997lasso}. 
In addition to the CoxPH model, deep learning methods have been developed for other survival models in the field of survival analysis. Among others, \cite{biganzoli1998feed} proposed a feedforward artificial neural networks (FFANNs) discrete logistic model. \cite{liestbl1994survival} developed a discrete time model with one hidden layer and a single output node for each subject. \cite{zhao2020deep,zhao2019dnnsurv} proposed deep neural networks based on pseudo values \cite{miller1974jackknife}. \cite{hu2021transformer} proposed a transformer-based deep survival model. Deep learning survival models have also been applied to specific medical settings, \cite[among others]{luck2017deep,yousefi2017predicting,lv2022transsurv}.


\paragraph{Counterfactual survival estimation.} 

\cite{robins1992recovery} introduced inverse probability of censoring weighting in the context of randomized controlled trials with dependent censoring. \cite{makuch1982adjusted} proposed to use conditional survival models to obtain counterfactual survival curves. Dragon-Net, an end-to-end procedure for predicting treatment and outcome models from confounders and treatment information, was developed by \cite{shi2019adapting}. \cite{shalit2017estimating} used a specific version of Dragon-Net TARNET as baseline. Other methods such as CEVAE \citep{louizos2017causal} and GANITE \citep{yoon2018ganite} utilize VAEs and GANs to estimate average treatment effects, respectively. Semiparametric efficient methods \citep{kennedy2022semiparametric} have also been proposed, \cite{hubbard2000nonparametric, bai2013doubly,westling2023inference}.


\paragraph{Debiased machine learning approaches and semi-parametric efficiency.} Debiased machine learning methods have been introduced across multiple disciplines such as biostatistics \citep{diaz2020machine}, econometrics, \citep{chernozhukov2022riesznet}, statistics \citep{kennedy2022semiparametric}, and computer science \cite{uehara2022review, kallus2020double}. The field of semiparametric efficient estimation is vast, with numerous notable contributions in the realm of causal inference, such as the works of \cite{kennedy2022semiparametric,diaz2020machine,chernozhukov2017double,chernozhukov2022riesznet,robins1992recovery, tsiatis2006semiparametric}. 
%The EIF has been derived in various ways, using the theory of augmented inverse probability weighted complete case \citep{robins1992recovery, tsiatis2006semiparametric}, or 

%\cite{shi2019adapting} developed Dragon-Net, an end-to-end procedure for %predicting treatment and outcome models from confounders and treatment %information. \cite{shalit2017estimating} used TARNET as baseline which is a %specific version of Dragon-Net. CEVAE \cite{louizos2017causal} and GANITE %\cite{yoon2018ganite} use VAEs, and GANs to estimate average treatment effects, %respectively. 

%Traditionally, Cox PH is the method of choice for survival analysis. There has recently a push in the machine learning community for more flexible model e.g. breaking the proportional hazard assumption and utilzing neural networks \khiem{cite a lot}. 

\paragraph{Covarate balancing.}
\textit{Non survival context:} In their work, \cite{imai2014covariate} introduced the Covariate Balancing Propensity Score (CBPS) method, which utilizes the generalized method of moments to estimate a logistic regression model for achieving covariate balance. \cite{fong2018covariate} extended CBPS to handle continuous treatments, which encompass measures of exposure or treatment intensity that are continuous in nature. Another approach, proposed by \cite{zubizarreta2015stable}, is the Stable Balancing Weights (SBW) method. SBW involves calculating a set of weights that minimize variance while satisfying a set of approximate moment matching conditions. \cite{hainmueller2012entropy} presented entropy balancing weights, which are obtained by minimizing the entropy of the weights while ensuring balance conditions are met. A weighted framework for estimating the effects of binary and continuous treatments was introduced by \cite{yiu2018covariate}, with connections established to the CBPS methodology. The literature on covariate balance is extensive, and numerous other methods have been developed for estimating the effect of binary treatments on continuous outcomes. Some notable examples include the works of \citep[among others]{kallus2021optimal,kallus2022optimal, kallus2021more,hirshberg2019minimax,hirshberg2021augmented,zhao2017entropy,zhao2019covariate,wong2017kernel,visconti2018handling,zubizarreta2014matching,li2018balancing,king2017balance,josey2020framework,yiu2018covariate}. Similarly, several approaches have been proposed to handle continuous treatments, such as those introduced by \citep[among others]{kallus2019kernel,tubbicke2020entropy,vegetabile2020nonparametric,wu2018matching,kennedy2017non}.

\textit{Survival context}: There is a limited body of research on covariate balance in the context of survival data. \cite{xue2023rkhs} built upon the work of \cite{wong2017kernel} and extended it to survival data by balancing covariates in a reproducing kernel Hilbert space (RKHS). \cite{abraich2022survcaus} expanded on the work of \cite{johansson2022generalization} to incorporate survival data. \cite{leete2019balanced} introduced a method that combines balanced policy evaluation with an imputation approach specifically designed for right-censored data. \cite{santacatterina2023robust} introduced weights that balance the correlation between confounders and a treatment.  \cite{yiu2022joint} extended the work of \cite{yiu2018covariate} to deal with censoring using marginal structural models. None of these methods, however, provide results on asymptotic normality, which allows for statistical inference, hypothesis testing, and the construction of confidence intervals.


%balancing rkhs, but not shown to be asymptocally normal: $O_p(ln n n^{-1/2})$ in sup norm
%Cross sectional context: efficiency shown for augmented balancing weights (AMLE, Hirshberg and Wager) and w/o augmentation (Minimax Linear Estimation of the Retargeted Mean, Hirshberg et al) 




%riesz representer (whitney locally robust semiparametric esetimation)

\paragraph{}

==> sections/relatedwork2.tex <==
\section{Related work}
\label{sec:related-work}
%We start by introducing standard counterfactual survival estimation methods, such as outcome regressions as proposed by \cite{makuch1982adjusted} and inverse probability weighting estimators as in \cite{robins1992recovery}. We then introduce an efficient influence function of the survival causal parameter of interest. Our proposed efficient influence function allows us to construct an efficient estimator in the spirit of debiased machine learning approaches that is also stable.
% Is EIF-based estimation a novelty here?

%\subsection{Non-efficient and efficient estimators}
%\subsection{Standard approaches and the efficient influence function.}
%From proposition~\ref{prop:identification}, a direct approach to estimating $\estimand^{a,t}$ is by estimating the event survival $S(t|a,X)$ conditional on the treatment and covariate

\paragraph{Outcome regression and inverse probability weighting estimators.} 
Based on Proposition~\ref{prop:identification}, the \textit{outcome regression} approach \citep{makuch1982adjusted} estimates $\psi^{a,t}$ is by directly estimating the conditional event survival $S_t(a,X)$ given the treatment and covariates. Parametric and semi-parametric models such as the Cox proportional hazard (CoxPH) model \citep{cox1972regression, andersen1982cox} in addition to deep learning techniques \citep{zhu2016deep,katzman2018deepsurv,faraggi1995neural,wang2021cox,ching2018cox,sun2020genome, zhong2022deep,nagpal2021deepcoxmixtures,meixide2022neural,lv2022transsurv,tibshirani1997lasso,biganzoli1998feed,liestbl1994survival,zhao2020deep,zhao2019dnnsurv,hu2021transformer,luck2017deep,yousefi2017predicting,lv2022transsurv} have been proposed to estimate $S_t(a,X)$.
A popular alternative to outcome regression is the inverse probability of censoring and treatment weighting estimator (IPW) \citep{robins1992recovery} defined as
$1 - \frac{1}{n}\sum_{i=1}^n \frac{\one(A_i=a)}{\hat \pi(X_i, a)}\frac{\one(E_i=1)}{\hat G_{T_i}(X_i, a)} \one(\td T_i \le t)$. In the past, model misspecification is a problem for both approaches. Modern machine learning methods can readily alleviate this, but they are data hungry, which motivates the use of semi-parametric efficient estimators \citep{chernozhukov2017double}.

\paragraph{Semi-parametric efficient estimators.}
The recent wake of big data and machine learning attracts renewed attention for the field of semi-parametric efficient estimation, with numerous notable contributions focusing on causal inference, such as \cite{diaz2020machine,chernozhukov2017double,chernozhukov2022riesznet,robins1992recovery, tsiatis2006semiparametric}. One starts from the efficient influence function (EIF), which determines the fastest rate of any \textit{regular} estimators \citep{van2000asymptotic}, and construct efficient estimators e.g. the one-step estimator \citep{kennedy2022semiparametric}. 
Similar EIFs to \ref{eq:eif} but with different parameterization are found in e.g. \citet{diaz2019statistical, cai2020one, hubbard2000nonparametric, bai2013doubly, bai2017optimal, westling2023inference}. All semi-parametric efficient estimators are the same asymptotically \citep{van2000asymptotic}, whose asymptotic variances are determined by the EIF, similar to Theorem \ref{thm:efficiency}; this key property shows that our estimator is asymptotically as good as other semi-parametric efficient ones. It does not, however, characterize an estimator's finite-sample behavior.

\paragraph{Covariate balancing.}
Numerous covariate balancing methods have been developed for estimating the effect of binary/continuous treatments on continuous outcomes including \citep[among others]{kallus2021optimal,kallus2022optimal, kallus2021more,hirshberg2019minimax,hirshberg2021augmented,zhao2017entropy,zhao2019covariate,wong2017kernel,visconti2018handling,zubizarreta2014matching,li2018balancing,king2017balance,josey2020framework,yiu2018covariate,hainmueller2012entropy,imai2014covariate,zubizarreta2015stable}. There is however limited body of research on covariate balance in the context of survival data \citep{xue2023rkhs,abraich2022survcaus,leete2019balanced,santacatterina2023robust,yiu2022joint,kallus2021optimal}. %\cite{xue2023rkhs} built upon the work of \cite{wong2017kernel} and extended it to survival data by balancing covariates in a reproducing kernel Hilbert space (RKHS). \cite{abraich2022survcaus} expanded on the work of \cite{johansson2022generalization} to incorporate survival data. \cite{leete2019balanced} introduced a method that combines balanced policy evaluation with an imputation approach specifically designed for right-censored data. \cite{santacatterina2023robust} introduced weights that balance the correlation between confounders and a treatment.  \cite{yiu2022joint} extended the work of \cite{yiu2018covariate} to deal with censoring using marginal structural models. 
Perhaps the most similar to our work and motivation is \citet{xue2023rkhs}, which is a covariate-balancing extension of \citet{xie2005adjusted}. Unfortunately, they assume independent censoring ($T$ and $C$ are independent unconditionally of $X$) and their estimator is inefficient. None of the mentioned covariate-balancing methods in survival context provide results on asymptotic normality like ours, which allows for statistical inference, hypothesis testing, and the construction of confidence intervals.




==> sections/trash.tex <==
% This is proven in the appendix. Note that the Riesz representation uses inverse probability weighting to replace evaluation of $\delta$ at $A=1$ with an inverse probability weighted indicator; in effect, the indicator identifies the correct population on which to evaluate $\delta$ ($1(E=1,A=1)\delta(A,X)=1(E=1,A=1)\delta(1,X)$) and weighting corrects for the population selection induced by this indicator. This is typical of Riesz representations in causal and missing data problems. 


% However, this Riesz representation cannot be used directly because it depends on the (unknown) inverse probability weights $\omega$; we must estimate it. One approach is to estimate the functions $\pi$ and $H$ and simply plug them in to the formula. Doing this yields the one-step estimator \citep[among others]{kennedy2022semiparametric,diaz2020machine,chernozhukov2017double}. However, these methods can be unstable in practice as they often involve estimating inversions (refer to Section \ref{sec:challenge} for more details).


\khiem{
maximizing $f_1(x_1) + f_2(x_2) + f_2(x_3)$. 
If we're doing it over the cube, that means we get to
maximize

We're going to get a term like this.

$$
\sum_i\sum_u \hat\gamma_{iu} (Y_{iu} - \lambda_{iu}). 
$$

If $\hat\gamma_{iu}$ is a function of $X$, $A$, $\one(\td T \ge u)$ like $\gamma$ itself, then these terms have mean zero. But if $\hat\gamma_{i1}$ depends on $\tilde T \ge 2$,
that's not true anymore. This means we can't set a weight using an optimization problem that observes future outcomes.

}

\khiem{(remove)
An implication of this structure is that 
if $\gamma(Z)$ is a vector valued function with the same structure, and we're interested in the 
dot product $\gamma(Z) \cdot \lambda(Z)$, then we can think of the vector of indicators 
$Y$ with elements $Y_u = \one(E=1, T=u)$ as a proxy for $\lambda$. 
In particular,
it is a proxy in the sense that $\gamma(Z) \cdot \lambda(Z)$ and $\gamma(Z) \cdot Y$ have the same 
expectation. This is an implication of the law of iterated expectations applied coordinatewise.
\begin{equation}
\label{eq:balance_ind}
\E [\gamma_u(Z) Y_u] 
= \E [\gamma_u(Z)] \E[ Y_u \mid Z^{u} ] 
= \E [\gamma_u(Z) \lambda_u(Z)]. 
\end{equation}
We will find this useful in the next section, 
where we discuss a generalization of a method for estimating functionals of conditional means $\mu(Z_i)=\E[Y_i \mid Z_i]$
of scalar valued random variables $Y$ to functionals of hazards. 
}



%The left-hand side has treatment $A$ and history $G$ set to $a$ and $1$ respectively. Therefore, to equate the 2 sides, $\gamma_u(X,A,G_u)$ must consist of factors $\hat r_u(X,a)\one(A=a, G_u=1)\omega_u(X,A,G_u)$ for some unknown $\omega$. This gives the right-hand side as
%\begin{equation}
%\begin{aligned}
%&\sum_{u \le t}\E\left[\hat r_u(X,a)\one(A=a,G_u=1)\omega_u(X,A,G_u) h_u(X,A,G_u)\right]\\
%&= \sum_{u \le t}\E\left[\hat r_u(X,a)\E[\one(A=a,G_u=1)|X]\omega_u(X,a,1) h_u(X,a,1)\right]\\
%\end{aligned}
%\end{equation}
%which shows that $\omega_u$ must be
%\begin{equation}\label{eq:omega}
%\omega_u(X, a) = \frac{1}{\E\left[\one(A=a, G_u=1)|X\right]} = \frac{1}{P(A=a, \td T \ge u|X)} = \frac{1}{H_{u-}(X,a)\pi(X,a)}
%\end{equation}
%($\omega_u(X,a)$ does not depend on $g_u$, which is set to 1 similar to the hazard). Part of our Riesz representer, the weight $\one(A=a, G_u=1)\omega_u(X, a)$ has the typical form of an inverse probability weight in causal and missing data problems. It uses the indicator $\one(A=1,G_u=1)$ to identify the correct population on which to evaluate $(\lambda_u - \hat\lambda_u)(X,A,G_u)$ and the weight $\omega_u$ to correct for the population selection induced by this indicator. The term $\hat r_u(X,a)$ is unique to our context - it captures the \textit{non-linear dependence} of $\psi^{a,t}$ on $\lambda$. Indeed $ \hat r = \partials{\lambda}\psi^{a,t}(\hat \lambda)$ is the vector of partial derivatives of $\psi^{a,t}$ with respect to $\lambda$ and evaluated at $\hat \lambda$. In this way, our parameter departs from the linear-functional causal parameters more commonly seen in the literature.



# introduction
%exploration of different causal parameters A more general strategy is to estimate 

%For instance, \cite{vansteelandt2022assumption} proposed an estimand that corresponds to the hazard ratio within the Cox model but also holds meaningful interpretations in scenarios where the Cox model assumptions are not satisfied. Other researchers have investigated different survival causal estimands such as the average survival effect, the residual average survival effect and the survival quantile effect \citep[among others]{mansourvar2016additive,mao2018propensity}.  


==> sections_arxiv_icml/abstract.tex <==
%WHY SHOULD YOU CARE ABOUT THIS PROBLEM
We study the problem of estimating the average survival causal effect, where the aim is to characterize the impact of an intervention on the average survival times of a population.
% 
% Historically, the most popular estimates have been based on parametric or semi-parametric (e.g. proportional hazards) models; however, these methods suffer from problematic levels of bias. 
Recently debiased machine learning approaches are becoming increasingly popular, especially in applications where the covariate-outcome relationship is highly non-linear. However, despite their appealing theoretical properties e.g. double robustness and asymptotic linearity, these estimators tend to be unstable because the debiasing step involves the use of the \emph{inverses} of small estimated probabilities---small errors in the estimated probabilities can result in huge changes in their inverses and therefore the resulting estimator. This problem is exacerbated in survival settings where probabilities are a product of treatment assignment and censoring probabilities.
%WHAT WE DID
%
We propose a kernel covariate balancing approach to estimating \textbf{both of these inverses at once} via the characterization of the Riesz representer of the parameter's derivative, sidestepping this problem. The result is an estimator that is stable in practice and enjoys many of the same theoretical properties. In particular, under overlap and asymptotic equicontinuity conditions, our estimator is asymptotically normal with negligible bias and optimal variance. % (this means it is not possible to do statistical inference better than ours)
%We introduce a covariate-balancing estimator that is both stable as well as asymptotically normal when the convergence rate of the nuisance estimators are at least $o(n^{-1/4})$.
%This assumption covers a broad range of machine learning methods, including neural networks.
%
%HOW IT WORKS
%Our proposed estimator is based on the efficient influence function of the treatment-specific survival curves, however we sidestep estimating the propensity weight directly, but estimate the balancing weight via a population balance property.
%
% EXPERIMENTS/THEORY TO BACK UP OUR STORY
Our experiments on synthetic and semi-synthetic data demonstrate that our method has competitive bias and smaller variance than debiased machine learning approaches. % because it is stable to extreme weights.
% We present experimental results on synthetic data that demonstrate the stability of our methods.






%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%NOTES


% However, the form of the semi-parametric efficient estimator involves inverse weights, which is unstable.?


% while the bias resulting from the incorrect misspecification of these models was small relative to the estimator's variance in yesterday's small sample sizes and therefore essentially unproblematic, it tends to be the dominant source of error in the larger samples we see today.

%in the large sample sizes we see today [the inability of these models to capture what the data tells us] is the dominant source 

%Existing methods for estimating survival causal effects [CITE Cox, IPCW] tend to suffer either from problematic levels of bias or instability. In particular, the theoretically optimal ... estimator involves the use of 

% Estimates based on parametric or semiparametric outcome models suffer from bias; it's possible to correct this bias using inverse probability weighting, but the resulting estimators suffer from instability due to the use of extreme (estimated) weights. In particular, while there is theory that tells us the essential form of the optimal estimator, it's very difficult to use in practice: it is highly sensitive to some parameters --- small probabilities --- that it requires us to estimate.

% use of this estimator requires us to estimate

% is known, practical ... lead to these instability problems. These ... are our focus. We propose ...

%but there are practical

%bias-corrected estimators exist, (especially using data-adaptive machine learning methods?), but suffer from instability due to the extreme weights required to render ... comparable.

% tend to require the estimation of large we the inverse 
% involve heavily weighting some observations, resulting in instability.


%estimation corrects for this, but 
%In particular, while the essential form of the optimal estimator is known, practical ... lead to these instability problems. These ... are our focus. We propose ...

%but there are practical


%leaves details to us that we usually screw up.

%times up to an event.

%times up to an event under

%probability of survival up to a given time under different treatments.  
%determine the impact of an intervention on the survival time. 





%arising from lack of overlap. 

%The standard approach of using inverse probability of treatment weighting can be sensitive to model misspecification and lead to high-variance estimates due to extreme weights.

%Survival causal effects are important because XXX, but %existing methods suffer either from lack of statistical %efficiency (like YYY) or from instability/high variance due to lack of %overlap (like inverse propensity weighting)

==> sections_arxiv_icml/abstract_2.tex <==
We study the problem of estimating the average survival causal effect, in particular the counterfactual survival curves, where the aim is to characterize the impact of an intervention on the survival times of a population.
% Debiased machine learning estimators for the counterfactual survival curves have been introduced that can incorporate flexible machine learning methods to capture complex covariate-outcome relationship while remaining asymptotically efficient. 
% However, they tend to be unstable because the debiasing step involves the use of the \emph{inverses} of small estimated probabilities. This problem is exacerbated in survival settings where probabilities are a product of treatment assignment and censoring probabilities.
We propose a kernel covariate balancing approach to the influence-function-based estimator of the counterfactual survival curves. Our approach estimates the inverses of small estimated probabilities in previous debiased machine learning approaches directly via the characterization of the Riesz representer of the parameter's derivative.
This helps us sidestep the inverse probability instability problem, which is exacerbated in survival settings where probabilities are a product of treatment assignment and at-risk probabilities.
The resulting estimator is stable in practice while still enjoys many of the same theoretical properties. In particular, under overlap and asymptotic equicontinuity conditions, our estimator is asymptotically efficient. Our experiments on synthetic and semi-synthetic data demonstrate that our method has competitive bias and smaller variance than previous inverse probability weight-based estimators.

==> sections_arxiv_icml/introduction_2.tex <==
\section{Introduction}
%\khiem{introduction (add intro plot here, terse description of data more detail in exp), setting (stastical, causal), approach(overlap challenge (add motivation plot here), AMLE, method), related work (refernces, OR and IPW, EIF), Theory and Implementation ?(asymptotic analysis, RKHS, survival estimation, bla), Experiment results.}

The estimation of the impact of interventions on survival times is a key objective in numerous studies, concerning drug efficacy's evaluation at ICU stay duration and assessment of advertising campaigns' effects on customer dwell time, etc. 

The predominant approach for assessing the impact of interventions on survival times is to employ the Cox proportional hazards model (CoxPH) \citep{cox1972regression, andersen1982cox}. This model estimates conditional hazard ratios, which serve as a measure of survival causal effects. However, the causal interpretation of conditional hazard ratios within the CoxPH model can be complex \citep{martinussen2022causality,vansteelandt2022assumption}. Hence, there has been a growing interest in directly estimating \textit{counterfactual survival curves} and consequently deriving survival causal effects from these estimates \citep{westling2023inference} such as the average survival effect, the residual average survival effect, and the survival quantile effect \citep{mansourvar2016additive, mao2018propensity}. A counterfactual survival curve represents the probability of an event occurring at a specific point in time, if contrary to fact, the entire population had undergone a specific intervention, given that the event of interest has not yet occurred. %Some commonly investigated survival causal effects include 

Traditional approaches for estimating counterfactual curves in survival analysis have relied on conditional parametric or semiparametric regression models \citep{kleinbaum2012parametric,cox1972regression}, or weighted methods based on inverse probability of censoring and treatment weighting (IPW) \citep{robins1992recovery}. However, both approaches can suffer from model misspecification i.e. the model does not contain the truth. Weighted methods are also susceptible to extreme inversions \citep{kang2007demystifying,kallus2022optimal,kallus2021more}. In recent years, debiased machine learning approaches have gained popularity due to their appealing double robustness property which deals with model misspecification in addition to being semiparametric efficient \citep{kennedy2022semiparametric}. Specifically, double robustness implies that even if only certain models that need to be estimated are correctly specified, these approaches remain consistent, ie., asymptotycally unbiased. Semiparametric efficiency refers to the ability of an estimator or estimation method to achieve the smallest possible \textit{asymptotic} variance among a class of semiparametric estimators. Despite their desirable theoretical properties, debiased machine learning methods \textit{still} face challenges associated with extreme inversions because they are necessarily characterized by inverse probability weights \citep{chernozhukov2022riesznet}.

Covariate balancing methods have been proposed as a solution to the issue of extreme weights encountered in other approaches \citep{ben2021balancing}. 
%TODO: refine (skip)
Instead of directly incorporating inverse probabilities, these methods employ a weight-learning process that yields more stable estimates while preserving crucial properties like semiparametric efficiency. However, the application of these methods to estimate survival causal effects has been significantly limited \citep{xue2023rkhs,wong2017kernel,abraich2022survcaus,johansson2022generalization,santacatterina2023robust,kallus2021optimal,yiu2022joint}, with none of them providing results on asymptotic normality. Asymptotic normality is crucial for statistical inference, hypothesis testing, and the construction of confidence intervals, highlighting a current gap in the literature.

Our main contribution to the literature of survival causal effects estimation is a novel approach based on covariate balancing techniques. It offers stability in practical applications, and when certain conditions such as overlap and asymptotic equicontinuity are met, it demonstrates asymptotic normality with minimal bias and optimal variance, i.e., statistically efficiency. We substantiate these claims both theoretically (Section \ref{sec:approach} and through experiments conducted on synthetic and semi-synthetic data (Section \ref{sec:experiments_details}. Proofs, additional experiments, and some technical details are deferred to appendices.

==> sections_arxiv_icml/relatedwork.tex <==
\section{Related work}
\label{sec:related-work}
%We start by introducing standard counterfactual survival estimation methods, such as outcome regressions as proposed by \cite{makuch1982adjusted} and inverse probability weighting estimators as in \cite{robins1992recovery}. We then introduce an efficient influence function of the survival causal parameter of interest. Our proposed efficient influence function allows us to construct an efficient estimator in the spirit of debiased machine learning approaches that is also stable.
% Is EIF-based estimation a novelty here?

%\subsection{Non-efficient and efficient estimators}
%\subsection{Standard approaches and the efficient influence function.}
%From proposition~\ref{prop:identification}, a direct approach to estimating $\estimand^{a,t}$ is by estimating the event survival $S(t|a,X)$ conditional on the treatment and covariate


